Markov Chain Score Ascent: A Unifying Framework of Variational Inference with Markovian Gradients

Minimizing the inclusive Kullback-Leibler (KL) divergence with stochastic gradient descent (SGD) is challenging since its gradient is defined as an integral over the posterior. Recently, multiple methods have been proposed to run SGD with biased gradient estimates obtained from a Markov chain. This paper provides the first non-asymptotic convergence analysis of these methods by establishing their mixing rate and gradient variance. To do this, we demonstrate that these methods-which we collectively refer to as Markov chain score ascent (MCSA) methods-can be cast as special cases of the Markov chain gradient descent framework. Furthermore, by leveraging this new understanding, we develop a novel MCSA scheme, parallel MCSA (pMCSA), that achieves a tighter bound on the gradient variance. We demonstrate that this improved theoretical result translates to superior empirical performance.

==> gp_table.tex <==

\begin{table*}
  \vspace{-0.2in}
  \centering
  \caption{Test Log Predictive Density on Gaussian Process Logistic Classification}\label{table:gp}
  \vspace{-0.05in}
  \setlength{\tabcolsep}{4pt}
  \begin{threeparttable}
  \begin{tabular}{lrrrrrr}
    \toprule
    & \multicolumn{1}{c}{\multirow{2}{*}{ELBO}} & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{pMCSA}}} & \multicolumn{1}{c}{\multirow{2}{*}{JSA}} & \multicolumn{1}{c}{\multirow{2}{*}{CIS}} & \multicolumn{1}{c}{\multirow{2}{*}{CIS-RB}} & \multicolumn{1}{c}{\multirow{2}{*}{SNIS}} \\
    & & \multicolumn{1}{c}{\textbf{(ours)}} & & & & \\
    \midrule
    \textsf{sonar} & {-0.69 {\scriptsize{\(\pm 0.00\)}}} & {\bf-0.68 {\scriptsize{\(\pm 0.00\)}}} & {\bf-0.68 {\scriptsize{\(\pm 0.00\)}}} & {\bf-0.68 {\scriptsize{\(\pm 0.00\)}}} & {\bf-0.68 {\scriptsize{\(\pm 0.00\)}}} & {-0.69 {\scriptsize{\(\pm 0.00\)}}} \\
    \textsf{ionosphere} & {-0.36 {\scriptsize{\(\pm 0.01\)}}} & {\bf-0.35 {\scriptsize{\(\pm 0.01\)}}} & {\bf-0.35 {\scriptsize{\(\pm 0.01\)}}} & {\bf-0.35 {\scriptsize{\(\pm 0.01\)}}} & {\bf-0.35 {\scriptsize{\(\pm 0.01\)}}} & {\bf-0.35 {\scriptsize{\(\pm 0.01\)}}} \\
    \textsf{breast} & {\bf-0.10 {\scriptsize{\(\pm 0.00\)}}} & {-0.11 {\scriptsize{\(\pm 0.01\)}}} & {-0.14 {\scriptsize{\(\pm 0.01\)}}} & {-0.14 {\scriptsize{\(\pm 0.00\)}}} & {-0.14 {\scriptsize{\(\pm 0.01\)}}} & {-0.14 {\scriptsize{\(\pm 0.01\)}}} \\
    \textsf{heart} & {-0.44 {\scriptsize{\(\pm 0.01\)}}} & {\bf-0.43 {\scriptsize{\(\pm 0.01\)}}} & {\bf-0.43 {\scriptsize{\(\pm 0.01\)}}} & {\bf-0.43 {\scriptsize{\(\pm 0.01\)}}} & {\bf-0.43 {\scriptsize{\(\pm 0.01\)}}} & {-0.44 {\scriptsize{\(\pm 0.01\)}}} \\
    \textsf{german} & {\bf-0.48 {\scriptsize{\(\pm 0.01\)}}} & {-0.49 {\scriptsize{\(\pm 0.01\)}}} & {-0.50 {\scriptsize{\(\pm 0.01\)}}} & {-0.50 {\scriptsize{\(\pm 0.01\)}}} & {-0.51 {\scriptsize{\(\pm 0.02\)}}} & {-0.49 {\scriptsize{\(\pm 0.01\)}}} \\
    \textsf{australian} & {\bf-0.21 {\scriptsize{\(\pm 0.01\)}}} & {\bf-0.21 {\scriptsize{\(\pm 0.01\)}}} & {\bf-0.21 {\scriptsize{\(\pm 0.01\)}}} & {\bf-0.21 {\scriptsize{\(\pm 0.01\)}}} & {-0.22 {\scriptsize{\(\pm 0.01\)}}} & {\bf-0.21 {\scriptsize{\(\pm 0.01\)}}} \\\bottomrule
  \end{tabular}
  \begin{tablenotes}
    \item[]{\footnotesize \(\pm\) denotes the 95\% bootstrap confidence intervals obtained from 20 repetitions.}
  \end{tablenotes}
  \end{threeparttable}
  \vspace{-0.15in}
\end{table*}

%%% Local Variables:
%%% TeX-master: "master"
%%% End:


==> illustration.tex <==

\section{Illustration of Different Schemes}\label{section:illustration}
\begin{figure}[H]
  \centering
  \subfloat[Joint Stochastic Approximation]{
    \includegraphics[scale=0.35]{figures/diagram_2.png}
  }
  \hspace{0.6in}
  \subfloat[Proposed Algorithm]{
    \includegraphics[scale=0.35]{figures/diagram_3.png}
  }
  \caption{}
\end{figure}


==> lemma_lipschitz.tex <==

%%% Local Variables:
%%% TeX-master: "master"
%%% End:


==> logistic_table.tex <==

\begin{table*}
  \vspace{-0.2in}
  \centering
  \caption{Classification Accuracy and Log Predictive Density on Logistic Regression Problems}\label{table:logistic}
  \vspace{-0.05in}
  \setlength{\tabcolsep}{3pt}
  \begin{threeparttable}
  \begin{tabular}{lcccccc}
    \toprule
     & \multicolumn{2}{c}{\textbf{\texttt{Pima Indians}}} & \multicolumn{2}{c}{\textbf{\texttt{heart disease}}} & \multicolumn{2}{c}{\textbf{\texttt{German credit}}} \\
    \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
    & Test Accuracy & Test LPD
    & Test Accuracy & Test LPD
    & Test Accuracy & Test LPD \\\midrule
    ELBO & \textbf{0.77 {\scriptsize(0.77, 0.77)}} & -0.53 {\scriptsize(-0.55, -0.51)} & 0.84 {\scriptsize(0.84, 0.84)} & \textbf{-0.40 {\scriptsize(-0.40, -0.39)}} & \textbf{0.77 {\scriptsize(0.77, 0.77)}} & -0.54 {\scriptsize(-0.58, -0.50)}  \\\arrayrulecolor{black!30}\midrule
    par.-IMH (ours) & \textbf{0.77 {\scriptsize(0.77, 0.77)}} & \textbf{-0.51 {\scriptsize(-0.51, -0.50)}} & \textbf{0.85 {\scriptsize(0.84, 0.85)}} & \textbf{-0.40 {\scriptsize(-0.40, -0.40)}} & \textbf{0.77 {\scriptsize(0.77, 0.77)}} & \textbf{-0.50 {\scriptsize(-0.50, -0.50)}} \\
    seq.-IMH & 0.67 {\scriptsize(0.65, 0.69)} & -0.71 {\scriptsize(-0.76, -0.65)} & 0.79 {\scriptsize(0.78, 0.80)} & -0.45 {\scriptsize(-0.46, -0.44)} & 0.76 {\scriptsize(0.76, 0.76)} & -0.51 {\scriptsize(-0.51, -0.51)} \\
    single-CIS & 0.69 {\scriptsize(0.67, 0.71)} & -0.68 {\scriptsize(-0.73, -0.62)} & 0.79 {\scriptsize(0.78, 0.80)} & -0.46 {\scriptsize(-0.48, -0.44)} & 0.76 {\scriptsize(0.75, 0.76)} & -0.51 {\scriptsize(-0.52, -0.51)} \\
    single-CISRB & 0.71 {\scriptsize(0.69, 0.72)} & -0.62 {\scriptsize(-0.67, -0.58)} & 0.80 {\scriptsize(0.79, 0.81)} & -0.44 {\scriptsize(-0.45, -0.43)} & 0.76 {\scriptsize(0.76, 0.76)} & -0.52 {\scriptsize(-0.52, -0.51)} \\
    single-HMC & 0.75 {\scriptsize(0.75, 0.75)} & -0.52 {\scriptsize(-0.53, -0.52)} & 0.80 {\scriptsize(0.79, 0.81)} & -0.45 {\scriptsize(-0.46, -0.44)} & \textbf{0.77 {\scriptsize(0.76, 0.77)}} & -0.61 {\scriptsize(-0.72, -0.49)} \\
    SNIS & 0.72 {\scriptsize(0.71, 0.72)} & -0.59 {\scriptsize(-0.61, -0.57)} & 0.78 {\scriptsize(0.77, 0.79)} & -0.46 {\scriptsize(-0.48, -0.45)} & 0.75 {\scriptsize(0.75, 0.76)} & -0.52 {\scriptsize(-0.52, -0.52)} \\\bottomrule
  \end{tabular}
  \begin{tablenotes}
    \item[]{\footnotesize \(\pm\) denotes the 95\% bootstrap confidence intervals obtained from 20 repetitions.}
  \end{tablenotes}
  \end{threeparttable}
  \vspace{-0.15in}
\end{table*}

%%% Local Variables:
%%% TeX-master: "master"
%%% End:


==> master-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndii}For notational convenience, we define the shorthand \begin {align*} \pi \left (\vz ^{(1:N)}\right ) = \pi \left (\vz ^{(1)}\right ) \, \pi \left (\vz ^{(2)}\right ) \times \ldots \times \pi \left (\vz ^{(N)}\right ). \end {align*} Then, \begin {alignat}{2} &\Esub {\Pi }{ f\left (\vlambda , \rvveta \right ) } \nonumber \\ &\quad = \int \left (- \frac {1}{N} \sum ^{N}_{n=1} \log q\left (\vz ^{(n)}; \vlambda \right ) - \mathbb {H}\left [\,\pi \,\right ]\right ) \, \pi \left (\vz ^{(1:N)}\right ) \, d\vz ^{(1:N)} \nonumber \\ &\quad = \int \left (- \frac {1}{N} \sum ^{N}_{n=1} \log q\left (\vz ^{(n)}; \vlambda \right )\right ) \, \pi \left (\vz ^{(1:N)}\right ) \, d\vz ^{(1:N)} - \mathbb {H}\left [\,\pi \,\right ] \nonumber \\ &\quad = \frac {1}{N} \sum ^{N}_{n=1} \left \{ \int \big (-\log q\,(\,\vz ^{(n)}; \vlambda \,)\,\big ) \, \pi \left (\vz ^{(1:N)}\right ) \, d\vz ^{(1:N)} \right \} - \mathbb {H}\,[\,\pi \,] \nonumber \\ &\quad = \frac {1}{N} \sum ^{N}_{n=1} \int \big ( -\log q\,(\,\vz ^{(n)}; \vlambda \,) \,\big ) \, \pi \left (\vz ^{(n)}\right ) \, d\vz ^{(n)} - \mathbb {H}\,[\,\pi \,] &&\quad {\text {\textit {Marginalized \(\vz ^{(m)}\) for all \(m \neq n\)}}} \nonumber \\ &\quad = \frac {1}{N} \sum ^{N}_{n=1} \int \big ( -\log q\,(\,\vz ^{(n)}; \vlambda \,) + \log \pi \left (\vz ^{(n)}\right ) \,\big ) \, \pi \left (\vz ^{(n)}\right ) \, d\vz ^{(n)} &&\quad {\text {\textit {Definition of \(\mathbb {H}\left [\pi \right ]\)}}} \nonumber \\ &\quad = \frac {1}{N} \sum ^{N}_{n=1} \int \pi \left (\vz ^{(n)}\right ) \, \log \frac {\pi \left (\vz ^{(n)}\right )}{q\,(\,\vz ^{(n)}; \vlambda \,)} \, d\vz ^{(n)} \nonumber \\ &\quad = \frac {1}{N} \sum ^{N}_{n=1} \DKL {\pi }{q\left (\cdot ; \vlambda \right )} \nonumber &&\quad {\text {\textit {Definition of \(d_{\text {KL}}\)}}} \\ &\quad = \DKL {\pi }{q\left (\cdot ; \vlambda \right )}.\label {eq:F_KL} \end {alignat} For \(\Esub {\Pi }{ \vg \left (\vlambda , \rvveta \right ) }\), note that \begin {align} \nabla _{\vlambda } f\left (\vlambda , \veta \right ) = -\frac {1}{N} \sum ^{N}_{n=1} \nabla _{\vlambda } \log q\left (\vz ^{(n)}; \vlambda \right ) = -\frac {1}{N} \sum ^{N}_{n=1} \vs \left (\vz ^{(n)}; \vlambda \right ) = \vg \left (\vlambda , \veta \right ).\label {eq:F_grad_G} \end {align} Therefore, it suffices to show that \begin {align*} \nabla _{\vlambda } \DKL {\pi }{q\left (\cdot ; \vlambda \right )} &= \nabla _{\vlambda } \Esub {\Pi }{ f\left (\vlambda , \rvveta \right ) } &&\text {\textit {\cref {eq:F_KL}}} \\ &= \Esub {\Pi }{ \nabla _{\vlambda } f\left (\vlambda , \rvveta \right ) } &&\text {\textit {{Leibniz derivative rule}}} \\ &= \Esub {\Pi }{ \vg \left (\vlambda , \rvveta \right ) }. &&\text {\textit {\cref {eq:F_grad_G}}} \end {align*}\end{proof}

\begin{restatable}[]{proposition}{prAtEndRestateiii}\label{thm:prAtEndiii}\label {thm:wstar} The maximum importance weight \(w^* = \sup _{\vz } w\left (\vz \right ) = \sup _{\vz } \pi \left (\vz \right )/q\left (\vz ;\vlambda \right )\) is bounded below exponentially by the KL divergence as \[ \exp \left ( \DKL {\pi }{q\left (\cdot ; \vlambda \right )} \right ) < w^*. \]\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndiii}\begin {alignat*}{2} \DKL {\pi }{q\left (\cdot ; \vlambda \right )} &= \Esub {\rvvz \sim \pi \left (\cdot \right )}{ \log \frac {\pi \left (\rvvz \right )}{q\left (\rvvz ; \vlambda \right )} } &&\quad \text {\textit {Definition of \(d_{\text {KL}}\)}} \\ &\leq \log \Esub {\rvvz \sim \pi \left (\cdot \right )}{ \frac {\pi \left (\rvvz \right )}{q\left (\rvvz ; \vlambda \right )} } &&\quad \text {\textit {Jensen's inequality}} \\ &\leq \log \Esub {\rvvz \sim \pi \left (\cdot \right )}{ w^* } \\ &= \log w^*. \end {alignat*}\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestateiv}\label{thm:prAtEndiv}\label {thm:product_measure_bound} For the probability measures \(p_1, \ldots , p_N\) and \(q_1, \ldots , q_N\) defined on a measurable space \((\mathsf {X}, \mathcal {A})\) and an arbitrary set \(A \in \mathcal {A}\), \begin {align*} &\abs { \int _{A^N} p_1\left (dx_1\right ) p_2\left (dx_2\right ) \times \ldots \times p_N\left (dx_N\right ) - q_1\left (dx_1\right ) q_2\left (dx_2\right ) \times \ldots \times q_N\left (dx_N\right ) } \\ &\qquad \leq \sum _{n=1}^N \abs { \int _{A} p_n\left (dx_n\right ) - q_n\left (dx_n\right ) } \end {align*}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndiv}By using the following shorthand notations \begin {alignat*}{2} p_{(1:N)}\left (dx_{(1:N)}\right ) &= p_1\left (dx_1\right ) p_2\left (dx_2\right ) \times \ldots \times p_N\left (dx_N\right ) \\ q_{(1:N)}\left (dx_{(1:N)}\right ) &= q_1\left (dx_1\right ) q_2\left (dx_2\right ) \times \ldots \times q_N\left (dx_N\right ), \end {alignat*} the result follows from induction as \begin {alignat}{2} &\abs { \int _{A^N} p_{(1:N)}\left (dx_{(1:N)}\right ) - q_{(1:N)}\left (dx_{(1:N)}\right ) } \nonumber \\ &\quad = \Bigg |\; \left ( \int _{A} p_1\left (dx_1\right ) - q_1\left (dx_1\right ) \right ) \, \int _{A^{N-1}} p_{(2:N)}\left (dx_{(2:N)}\right ) \nonumber \\ &\qquad \quad + \int _{A} q_1\left (dx_1\right ) \, {\left ( \int _{A^{N-1}} p_{(2:N)}\left (dx_{(2:N)}\right ) - q_{(2:N)}\left (dx_{(2:N)}\right ) \right )} \;\Bigg | \nonumber \\ &\quad \leq \Bigg | \int _{A} p_1\left (dx_1\right ) - q_1\left (dx_1\right ) \Bigg |\; \int _{A^{N-1}} p_{(2:N)}\left (dx_{(2:N)}\right ) \nonumber \\ &\qquad \quad + \int _{A} q_1\left (dx_1\right ) \, { \Bigg |\; \int _{A^{N-1}} p_{(2:N)}\left (dx_{(2:N)}\right ) - q_{(2:N)}\left (dx_{(2:N)}\right ) } \;\Bigg | &&\quad \text {\textit {Triangle inequality}} \nonumber \\ &\quad \leq \Bigg | \int _{A} p_1\left (dx_1\right ) - q_1\left (dx_1\right ) \Bigg |\; \nonumber \\ &\qquad \quad + { \Bigg |\; \int _{A^{N-1}} p_{(2:N)}\left (dx_{(2:N)}\right ) - q_{(2:N)}\left (dx_{(2:N)}\right ) } \;\Bigg |. &&\quad \text {\textit {Applied \(p_n\left (A\right ), q_n\left (A\right ) \leq 1 \)}} \nonumber \end {alignat}\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatev}\label{thm:prAtEndv}\label {thm:second_moment_bound} Let \(\rvvg \) be a vector-valued, biased estimator of \(\vmu \), where the bias is denoted as \(\mathsf {Bias}\left [\rvvg \right ] = \norm { \mathbb {E}\rvvg - \vmu }_2\) and the mean-squared error is denoted as \(\mathsf {MSE}\left [\rvvg \right ] = \mathbb {E}\norm {\rvvg - \vmu }_2^2\). Then, the second moment of \(\rvvg \) is bounded as \begin {enumerate} \item [\ding {182}] \( \mathbb {E}\norm {\rvvg }^2_2 \leq \mathbb {V}{\rvvg } + {\mathsf {Bias}\left [\rvvg \right ]}^2 + 2\, \mathsf {Bias}\left [\rvvg \right ] \norm {\vmu }_2 + \norm {\vmu }^2_2, \) \item [\ding {183}] \( \mathbb {E}\norm {\rvvg }^2_2 \leq \mathsf {MSE}\left [{\rvvg }\right ] + 2\, \mathsf {Bias}\left [\rvvg \right ] \norm {\vmu }_2 + \norm {\vmu }^2_2, \) \end {enumerate} where \(\mathbb {V}\rvvg = \mathbb {E}\norm { \rvvg - \mathbb {E}\vg }_2^2\) is the variance of the estimator.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndv}\ding {182} follows from the decomposition {\begin {alignat}{2} \E { \norm {\rvvg }^2_{2} } &\;= \mathbb {V}{ \rvvg } + \norm { \mathbb {E}{ \rvvg } }_2^2 \nonumber \\ &\;= \mathbb {V}{ \rvvg } + \norm { \mathbb {E}{ \rvvg } - \vmu + \vmu }_2^2 \nonumber \\ &\;= \mathbb {V}{ \rvvg } + \norm { \mathbb {E}{ \rvvg } - \vmu }_2^2 \nonumber + 2 \, {\left ( \mathbb {E}\rvvg - \vmu \right )}^{\top } \vmu + \norm {\vmu }^2_2 &&\quad \text {\textit {Expanded quadratic}} \nonumber \\ &\;\leq \mathbb {V}{ \rvvg } + \norm { \mathbb {E}{ \rvvg } - \vmu }_2^2 + 2 \,\norm { \mathbb {E}{ \rvvg } - \vmu }_2 \norm {\vmu }_2 + \norm { \vmu }_2^2 \nonumber &&\quad \text {\textit {Cauchy-Shwarz inequality}} \\ &\;= \mathbb {V}{ \rvvg } + {\mathsf {Bias}\left [\rvvg \right ]}^2 + 2 \,\mathsf {Bias}\left [\rvvg \right ] \norm {\vmu }_2 + \norm { \vmu }_2^2. \nonumber &&\quad \text {\textit {Definition of bias}} \end {alignat} } Meanwhile, by the well-known bias-variance decomposition formula of the mean-squared error, \ding {183} directly follows from \ding {182}.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndvi}MSC is described in~\cref {alg:msc}. At each iteration, it performs a single MCMC transition with the CIS kernel where it internally uses \(N\) proposals. That is, \begin {align*} \rvvz _t \mid \rvvz _{t-1}, \rvvlambda _{t-1} &\sim K_{\rvvlambda _{t-1}}\left (\rvvz _{t-1}, \cdot \right ) \\ \rvvg _{t,\text {MSC}} &= -\vs \left (\vlambda , \rvvz _t\right ), \end {align*} where \(K_{\rvvlambda _{t-1}}\) is the CIS kernel using \(q_{\text {def.}}\left (\cdot ; \rvvlambda _{t-1}\right )\). \par \paragraph {Ergodicity of the Markov Chain} The ergodic convergence rate of \(P_{\vlambda }\) is equal to that of \(K_{\vlambda }\), the CIS kernel proposed by~\citet {NEURIPS2020_b2070693}. Although not mentioned by~\citet {NEURIPS2020_b2070693}, this kernel has been previously proposed as the iterated sequential importance resampling (i-SIR) by \citet {andrieu_uniform_2018} with its corresponding geometric convergence rate as \begin {alignat*}{2} \DTV {P^{k}_{\vlambda }\left (\veta , \cdot \right )}{\Pi } = \DTV {K^{k}_{\vlambda }\left (\vz , \cdot \right )}{\pi } \leq {\left (1 - \frac {N - 1}{2 w^* + N - 2}\right )}^k. \end {alignat*} \par \paragraph {\textbf {Bound on the Gradient Variance}} The bound on the gradient variance is straightforward given \cref {thm:bounded_score}. For simplicity, we denote the rejection state as \(\vz ^{(1)}_t = \vz _{t-1} \). Then, \begin {alignat}{2} &\E { {\lVert \rvvg _{t,\text {MSC}}\rVert }^2 \,\middle |\, \mathcal {F}_{t-1} } \nonumber \\ &\;= \Esub {\rvvz _t \sim K_{\rvvlambda _{t-1}}\left (\rvvz _{t-1}, \cdot \right )}{ \norm { \vs \left (\vlambda ; \rvvz _t\right ) }^2 \,\middle |\, \rvvlambda _{t-1}, \rvvz _{t-1} } \nonumber \\ &\;= \int \sum ^{N}_{n=1} \frac { w\left (\vz ^{(n)}_t\right ) }{ \sum ^{N}_{m=1} w\left (\vz ^{(m)}_t\right ) } \norm { \vs \left (\vlambda ; \vz ^{(n)}_t\right ) }^2 \prod ^{N}_{n=2} q\left (d\vz ^{(n)}_t; \rvvlambda _{t-1}\right ) \nonumber &&\quad \text {\textit {\citet {andrieu_uniform_2018}}} \\ &\;\leq L^2 \, \int \sum ^{N}_{n=1} \frac { w\left (\vz ^{(n)}_t\right ) }{ \sum ^{N}_{m=1} w\left (\vz ^{(m)}_t\right ) } \prod ^{N}_{n=2} q\left (d\vz ^{(n)}_t; \rvvlambda _{t-1}\right ) \nonumber &&\quad \text {\textit {\cref {thm:bounded_score}}} \\ &\;= L^2 \, \int \prod ^{N}_{n=2} q\left (d\vz ^{(n)}; \rvvlambda _{t-1}\right ) \nonumber \\ &\;= L^2. \nonumber \end {alignat} \par \end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {thm:iw_variance} Let the importance weight be defined as \(w\left (\vz \right ) = \pi \left (\vz \right )/q\left (\vz \right )\). The variance of the importance weights is related to the \(\chi ^2\) divergence as \begin {align*} \mathbb {V}_{q}{w\left (\rvvz \right )} = \DChi {\pi }{q}. \end {align*}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndvii}{ \begin {alignat}{2} \mathbb {V}_{q}{w\left (\rvvz \right )} = \Esub {q}{ {\left ( w\left (\rvvz \right ) - \Esub {q}{ w\left (\rvvz \right ) } \right )}^2 } = \Esub {q}{ {\left ( w\left (\rvvz \right ) - 1 \right )}^2 } = \int {\left ( \frac {\pi \left (\vz \right )}{q\left (\vz \right )} - 1 \right )}^2 q\left (d\vz \right ) = \DChi {\pi }{q}. \nonumber \end {alignat} }\end{proof}

\prAtEndRestateviii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndviii}Rao-Blackwellization of the CIS kernel is to reuse the importance weights \(w\left (\vz \right ) = \pi \left (\vz \right ) / q_{\text {def.}}\left (\vz \right )\) internally used by the kernel when forming the estimator. That is, the gradient is estimated as \begin {align*} &\rvvz ^{(n)}_t \mid \rvvlambda _{t-1} \sim q\left (\cdot ; \rvvlambda _{t-1}\right ) \\ &\rvvg _{t,\text {MSC-RB}} = -\sum ^{N}_{n=2} \frac {w\left (\rvvz ^{(n)}_t\right )}{\sum ^{N}_{m=2}w\left (\rvvz ^{(n)}_t\right ) + w\left (\rvvz _{t-1}\right )} \vs \left (\rvvz ^{(n)}_t\right ) + \frac {w\left (\rvvz _{t-1}\right )}{\sum ^{N}_{m=2}w\left (\rvvz ^{(n)}_t\right ) + w\left (\rvvz _{t-1}\right )} \vs \left (\rvvz _{t-1}\right ). \end {align*} \par By \cref {thm:second_moment_bound}, the second moment of the gradient is bounded as \begin {alignat}{2} \E { {\parallel \rvvg _{t,\text {MSC-RB}} \parallel }_2^2 \,\middle |\, \mathcal {F}_{t-1} } &= \mathsf {MSE}\left [ \rvvg _{t, \text {MSC-RB}} \,\middle |\, \mathcal {F}_{t-1} \right ] + 2 \, {\mathsf {Bias}\left [ \rvvg _{t, \text {MSC-RB}} \,\middle |\, \mathcal {F}_{t-1} \right ]}^{\top } \norm {\vmu }_2 + \norm {\vmu }^2_2 \nonumber \\ &\leq \mathsf {MSE}\left [ \rvvg _{t, \text {MSC-RB}} \,\middle |\, \mathcal {F}_{t-1} \right ] + 2 \, L \, {\mathsf {Bias}\left [ \rvvg _{t, \text {MSC-RB}} \,\middle |\, \mathcal {F}_{t-1} \right ]} + \norm {\vmu }^2_2. \label {eq:mscrb_decomp} \end {alignat} \par \citet [Theorem 3]{cardoso_brsnis_2022} show that the mean-squared error of this estimator, which they call bias reduced self-normalized importance sampling, is bounded as \begin {align*} \mathsf {MSE}\left [ \rvvg _{t,\text {MSC-RB}} \,\middle |\, \mathcal {F}_{t-1} \right ] \leq 4\,L^2 \, \Big [\,& \left ( 1 + \epsilon ^2 \right )\, \frac {1}{N-1}\,\Vsub {\rvvz \sim q_{\text {def.}}\left (\cdot ; \rvvlambda _{t-1}\right )}{w\left (\rvvz \right ) \mid \rvvlambda _{t-1}} \\ &+ \left (1 + \epsilon ^{-2} \right )\, \frac {1}{N^2} {\left (1 + w^*\right )}^2 \,\Big ], \end {align*} for some arbitrary constant \(\epsilon ^2\). The first term is identical to the variance of an \(N-1\)-sample self-normalized importance sampling estimator~\citep {10.1214/17-STS611}, while the second term is the added variance due to ``rejections.'' \par Since the variance of the importance weights is well known to be related to the \(\chi ^2\) divergence, \begin {alignat}{2} \mathsf {MSE}\left [ \rvvg _{t,\text {MSC-RB}} \,\middle |\, \mathcal {F}_{t-1} \right ] \leq 4\,L^2 \, \Big [\,& \left ( 1 + \epsilon ^2 \right )\, \frac {1}{N-1}\,\DChi {\pi }{q\left (\cdot ; \rvvlambda _{t-1}\right )} \nonumber \\ &+ \left (1 + \epsilon ^{-2} \right )\, \frac {1}{N^2} {\left (1 + w^*\right )}^2 \,\Big ]. &&\quad \text {\textit {\cref {thm:iw_variance}}} \nonumber \end {alignat} \par For \(\epsilon ^2\), \citeauthor {cardoso_brsnis_2022} choose \(\epsilon ^2 = {\left (N-1\right )}^{-1/2}\), which results in their stated bound \begin {align*} \mathsf {MSE}\left [ \rvvg _{t,\text {MSC-RB}} \,\middle |\, \mathcal {F}_{t-1} \right ] \leq 4\,L^2 \, \Big [\, \frac {1}{N-1}\,\DChi {\pi }{q\left (\cdot ; \rvvlambda _{t-1}\right )} + \mathcal {O}\left (N^{-3/2}\right ) \,\Big ]. \end {align*} \par Furthermore, they show that the bias term is bounded as \begin {align*} \mathsf {Bias}\left [ \rvvg _{t,\text {MSC-RB}} \right ] \leq \frac {4 \, L}{N-1} \left ( \DChi {\pi }{q\left (\cdot ; \rvvlambda _{t-1}\right )} + 1 + w^*\right ) {\left ( \frac {2 w^*}{ 2 w^* + N - 2 } \right )}^{t-1}. \end {align*} Combining both the bias and the mean-squared error to \cref {eq:mscrb_decomp}, we obtain the bound \begin {align*} &\E { {\lVert \rvvg _{t,\text {MSC-RB}} \rVert }_2^2 \,\middle |\, \mathcal {F}_{t-1} } \\ &\;\leq 4\,L^2\,\bigg [ \frac {1}{N-1}\,\DChi {\pi }{q\left (\cdot ; \rvvlambda _{t-1}\right )} \\ &\qquad + \frac {1}{N-1} \left ( \DChi {\pi }{q\left (\cdot ; \rvvlambda _{t-1}\right )} + 1 + w^*\right ) {\left ( \frac {2 w^*}{ 2 w^* + N - 2 } \right )}^{t-1} + \mathcal {O}\left (N^{-3/2}\right ) \bigg ] \\ &= 4 \, L^2 \,\bigg [ \frac {1 + \gamma ^{t-1}}{N-1}\,\DChi {\pi }{q\left (\cdot ; \rvvlambda _{t-1}\right )} + \frac {\gamma ^{t-1}}{N-1} + \frac {\gamma ^{t-1} w^*}{N-1} + \mathcal {O}\left (N^{-3/2}\right ) \bigg ]. \end {align*}\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestateix}\label{thm:prAtEndix}\label {thm:lambda_bound} For \(w^* = \sup _{\vz } w\left (\vz \right ) \), \(\lambda \left (\cdot \right )\) in~\cref {eq:T_lambda} is bounded as \[ \max \left (1 - \frac {1}{w}, 0\right ) \leq \lambda \left (w\right ) \leq 1 - \frac {1}{w^*}. \]\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndix}The proof can be found in the proof of Theorem 3 of \citet {Smith96exacttransition}.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatex}\label{thm:prAtEndx}\label {thm:tn_bound} For \(w^* = \sup _{\vz } w\left (\vz \right ) \), \(T_n\left (\cdot \right )\) in~\cref {eq:T_lambda} is bounded as \[ T_n\left ( w \right ) \leq \frac {n}{w} \, {\left (1 - \frac {1}{w^*}\right )}^{n-1}. \]\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndx}\begin {alignat*}{2} T_n\left (w\right ) &= \int _w^{\infty } \frac {n}{v^2} \, \lambda ^{n-1}\left (v\right )\,dv &&\quad \text {\textit {\cref {eq:T_lambda}}} \\ &\leq \int _w^{\infty } \frac {n}{v^2} \, {\left (1 - \frac {1}{w^*}\right )}^{n-1}\,dv &&\quad \text {\textit {\cref {thm:lambda_bound}}} \\ &= n \, {\left (1 - \frac {1}{w^*}\right )}^{n-1} \int _w^{\infty } \frac {1}{v^2} \,dv \\ &= n \, {\left (1 - \frac {1}{w^*}\right )}^{n-1} \left ( {-\left .\frac {1}{v}\right \rvert ^{\infty }_{w}} \right ) \\ &= \frac {n}{w} \, {\left (1 - \frac {1}{w^*}\right )}^{n-1}. \end {alignat*}\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexi}\label{thm:prAtEndxi}\label {thm:imh_expecation} For a positive test function \(f : \mathcal {Z} \rightarrow \mathbb {R}^{+}\), the estimate of a \(\pi \)-invariant independent Metropolis-Hastings kernel \(K\) with a proposal \(q\) is bounded as \begin {align*} \Esub {K^n\left (\vz , \cdot \right )}{ f \,\middle |\, \rvvz } \leq n \, r^{n-1} \Esub {q}{f} + {r}^n \, f\left (\rvvz \right ), \end {align*} where \(w\left (\vz \right ) = \pi \left (\vz \right ) / q\left (\vz \right )\) and \(r = 1 - \nicefrac {1}{w^*}\) for \(w^* = \sup _{\vz } w\left (\vz \right ) \).\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxi}\begin {alignat*}{2} &\Esub {K^n\left (\vz , \cdot \right )}{ f \,\middle |\, \vz } \\ &\quad = \int T_n\left (w\left (\vz \right ) \vee w\left (\vz ^{\prime }\right )\right ) \, f\left (\vz ^{\prime }\right ) \, \pi \left (\vz ^{\prime }\right ) d\vz ^{\prime } + \lambda ^{n}\left (w\left (\rvvz \right )\right ) \, f\left (\rvvz \right ) &&\quad {\text {\textit {\cref {eq:imh_exact_kernel}}}} \\ &\quad \leq \int \frac {n}{w\left (\vz \right ) \vee w\left (\vz ^{\prime }\right )} \, {\left (1 - \frac {1}{w^*}\right )}^{n-1} \, f\left (\vz ^{\prime }\right ) \, \pi \left (\vz ^{\prime }\right ) d\vz ^{\prime } + \lambda ^{n}\left (w\left (\rvvz \right )\right ) \, f\left (\rvvz \right ) &&\quad {\text {\textit {\cref {thm:tn_bound}}}} \\ &\quad \leq \int \frac {n}{w\left (\vz ^{\prime }\right )} \, {\left (1 - \frac {1}{w^*}\right )}^{n-1} \, f\left (\vz ^{\prime }\right ) \, \pi \left (\vz ^{\prime }\right ) d\vz ^{\prime } + \lambda ^{n}\left (w\left (\rvvz \right )\right ) \, f\left (\rvvz \right ) &&\quad {\frac {1}{w\left (\vz \right ) \vee w\left (\vz ^{\prime }\right )} \leq \frac {1}{w\left (\vz ^{\prime }\right )}} \\ &\quad = n \, {\left (1 - \frac {1}{w^*}\right )}^{n-1} \, \int \frac {1}{w\left (\vz ^{\prime }\right )} \, f\left (\vz ^{\prime }\right ) \, \pi \left (\vz ^{\prime }\right ) d\vz ^{\prime } + \lambda ^{n}\left (w\left (\rvvz \right )\right ) \, f\left (\rvvz \right ) \\ &\quad = n \, {\left (1 - \frac {1}{w^*}\right )}^{n-1} \, \int f\left (\vz ^{\prime }\right ) \, q\left (\vz ^{\prime }\right ) d\vz ^{\prime } + \lambda ^{n}\left (w\left (\rvvz \right )\right ) \, f\left (\rvvz \right ) &&\quad {\text {\textit {Definition of \(w\left (\vz \right )\)}}} \\ &\quad \leq n \, {\left (1 - \frac {1}{w^*}\right )}^{n-1} \, \int f\left (\vz ^{\prime }\right ) \, q\left (\vz ^{\prime }\right ) d\vz ^{\prime } + {\left (1 - \frac {1}{w^*}\right )}^{n} \, f\left (\rvvz \right ) &&\quad {\text {\textit {\cref {thm:lambda_bound}}}} \\ &\quad = n \, {\left (1 - \frac {1}{w^*}\right )}^{n-1} \Esub {q}{f} + {\left (1 - \frac {1}{w^*}\right )}^n \, f\left (\rvvz \right ). \end {alignat*}\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexii}\label{thm:prAtEndxii}\label {thm:mcmc_bias} Let a \(\Pi \)-invariant Markov chain kernel \(P\) be geometrically ergodic as \begin {align*} \DTV {P^{n}\left (\veta _0, \cdot \right )}{ \Pi } \leq C \, \rho ^{n}. \end {align*} Furthermore, let \(\widehat {\rvvg } = \vg \left (\rvveta \right )\) with \(\rvveta \sim P^n\left (\veta _0, \cdot \right )\) be the estimator of \(\mathbb {E}_{\Pi }\rvvg \) for some function \(\vg : \mathrm {H} \rightarrow \mathbb {R}^{D}\) bounded as \( \norm {\rvvg }_{2} \leq L \). The bias of \(\rvvg \), defined as \( \mathsf {Bias}\left [ \widehat {\rvvg } \right ] = \mathbb {E}\parallel \widehat {\rvvg } - \mathbb {E}_{\pi }\rvvg \parallel \), is bounded as \begin {alignat*}{2} \mathsf {Bias}\left [ \hat {\rvvg } \right ] \leq 2 \, \sqrt {D} \, L \, C \, \rho ^{n}. \end {alignat*}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxii}\begin {alignat}{2} \mathsf {Bias}\left [ \hat {\rvvg } \right ] &= \norm { \mathbb {E}_{P^n\left (\veta _0, \cdot \right )}\vg - \mathbb {E}_{\Pi }\vg }_2 \nonumber \\ &\leq \sqrt {D}\,\norm { \mathbb {E}_{P^n\left (\veta _0, \cdot \right )}\vg - \mathbb {E}_{\Pi }\vg }_{\infty } &&\quad \text {\textit {for \(\vx \in \mathbb {R}^D\), \(\norm {\vx }_2 \leq \sqrt {D}\norm {\vx }_{\infty }\)}} \nonumber \\ &\leq \sqrt {D}\,L\,\sup _{\abs {h} \leq 1} \abs { \mathbb {E}_{P^n\left (\veta _0, \cdot \right )}h - \mathbb {E}_{\Pi }h } &&\quad \text {\textit {\(\norm {\vg }_{\infty } \leq \norm {\vg }_2 \leq L\)}} \nonumber \\ &= 2 \, \sqrt {D} \, L \, \DTV {P^{n}\left (\veta ^{(0)}, \cdot \right )}{\pi } &&\quad \text {\textit {Definition of \(d_{\mathrm {TV}}\)}} \nonumber \\ &= 2 \, \sqrt {D} \, L \, C \, \rho ^{n}. &&\quad \text {\textit {Geometric ergodicity}} \nonumber \end {alignat}\end{proof}

\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxiii}\par JSA is described in~\cref {alg:jsa}. At each iteration, it performs \(N\) MCMC transitions and uses the \(N\) intermediate states to estimate the gradient. That is, \begin {align*} \rvvz ^{(1)}_{t} &\mid \rvvz _{t-1}^{(N)},\, \rvvlambda _{t-1} \sim K_{\rvvlambda _{t-1}}\left (\rvvz _{t-1}^{(N)}, \cdot \right ) \\ \rvvz ^{(2)}_{t} &\mid \rvvz ^{(1)}_{t},\, \rvvlambda _{t-1} \sim K_{\rvvlambda _{t-1}}\left (\rvvz _{t}^{(1)}, \cdot \right ) \\ &\qquad \qquad \vdots \\ \rvvz ^{(N)}_{t} &\mid \rvvz ^{(N-1)}_{t},\, \rvvlambda _{t-1} \sim K_{\rvvlambda _{t-1}}\left (\rvvz _{t}^{(N-1)}, \cdot \right ) \\ \rvvg _{t,\text {JSA}} &= -\frac {1}{N}\,\sum ^{N}_{n=1} \, \vs \left (\vlambda , \rvvz ^{(n)}_t\right ), \end {align*} where \(K_{\rvvlambda _{t-1}}^n\) is an \(n\)-transition IMH kernel using \(q_{\text {def.}}\left (\cdot ; \rvvlambda _{t-1}\right )\). Under \cref {thm:bounded_weight}, an IMH kernel is uniformly geometrically ergodic~\citep {10.2307/2242610, wang_exact_2022} as \begin {align} \DTV {K_{\vlambda }^k\left (\vz , \cdot \right )}{\pi } \leq r^{k}\label {eq:imh_ergodicity} \end {align} for any \(\vz \in \mathcal {Z}\). \par \paragraph {Ergodicity of the Markov Chain} The state transitions of the Markov chain samples \(\vz ^{(1:N)}\) are visualized as {\small \begin {center} \bgroup \setlength {\tabcolsep }{3pt} \def \arraystretch {1.8} \begin {tabular}{c|ccccc} & \(\vz ^{(1)}_t\) & \(\vz ^{(2)}_t\) & \(\vz ^{(3)}_t\) & \(\ldots \) & \(\vz ^{(N)}_t\) \\ \midrule \(t=1\) & \(K_{\vlambda _1}\left (\vz _0, d\vz _1^{(1)}\right )\) & \(K_{\vlambda _1}^2\left (\vz _0, d\vz _1^{(2)}\right )\) & \(K_{\vlambda _1}^3\left (\vz _0, d\vz _1^{(3)}\right )\) & \(\ldots \) & \(K_{\vlambda _1}^N\left (\vz _0, d\vz _1^{(N)}\right )\) \\ \(t=2\) & \(K_{\vlambda _2}^{N + 1}\left (\vz _0, d\vz _2^{(1)}\right )\) & \(K_{\vlambda _2}^{N + 2}\left (\vz _0, d\vz _2^{(2)}\right )\) & \(K_{\vlambda _2}^{N + 3}\left (\vz _0, d\vz _2^{(3)}\right )\) & \(\ldots \) & \(K_{\vlambda _2}^{2\,N}\left (\vz _0, d\vz _2^{(N)}\right )\) \\ \(\vdots \) & & & \(\vdots \) & & \\ \(t=k\) & \(K_{\vlambda _k}^{\left (k-1\right )\,N + 1}\left (\vz _0, d\vz _k^{(1)}\right )\) & \(K_{\vlambda _k}^{\left (k-1\right )\,N + 2}\left (\vz _0, d\vz _k^{(2)}\right )\) & \(K_{\vlambda _k}^{\left (k-1\right )\,N + 3}\left (\vz _0, d\vz _k^{(3)}\right )\) & \(\ldots \) & \(K_{\vlambda _k}^{\left (k-1\right )\,N + N}\left (\vz _0, d\vz _k^{(N)}\right )\) \\ \end {tabular} \egroup \end {center} } where \(K_{\vlambda }\left (\vz , \cdot \right )\) is an IMH kernel. Therefore, the \(n\)-step transition kernel for the vector of the Markov-chain samples \(\veta = \vz ^{(1:N)}\) is represented as \begin {align*} P_{\vlambda }^k\left (\veta , d\veta ^{\prime }\right ) = K_{\vlambda }^{N\,\left (k-1\right ) + 1}\left (\vz _1, d\vz ^{\prime }_1\right ) \, K_{\vlambda }^{N\,\left (k-1\right ) + 2}\left (\vz _2, d\vz ^{\prime }_2\right ) \cdot \ldots \cdot K_{\vlambda }^{N\,\left (k-1\right ) + N}\left (\vz _N, d\vz ^{\prime }_N\right ). \end {align*} \par Now, the convergence in total variation \(d_{\mathrm {TV}}\left (\cdot , \cdot \right )\) can be shown to decrease geometrically as \begin {alignat}{2} &\DTV {P_{\vlambda }^{k}\left (\veta , \cdot \right )}{\Pi } \nonumber \\ &\quad = \sup _{A} \abs { \Pi \left (A\right ) - P^{k}\left (\veta , A\right ) } \nonumber \\ &\quad \leq \sup _{A} \Bigg | \int _{A} \pi \left (d\vz ^{\prime \;(1)}\right ) \times \ldots \times \pi \left (d\vz ^{\prime \;(N)}\right ) \nonumber &&\quad \text {\textit {Definition of \(d_{\text {TV}}\)}} \\ &\qquad \qquad \qquad - K^{(k-1)\,N\,+1}_{\vlambda }\left (\vz ^{(1)}, d\vz ^{\prime \;(1)}\right ) \times \ldots \times K^{k\,N}_{\vlambda }\left (\vz ^{(N)}, d\vz ^{\prime \;(N)}\right ) \,\Bigg | \nonumber \\ &\quad \leq \sup _{A} \sum _{n=1}^N \abs { \int _{A} \pi \left (d\vz ^{(n)}\right ) - K^{(k-1)\,N + n}_{\vlambda }\left (\vz ^{(n)}, d\vz ^{\prime \;(n)}\right ) } &&\quad \text {\textit {\cref {thm:product_measure_bound}}} \nonumber \\ &\quad = \sum _{n=1}^N \DTV {K^{(k-1)\,N + n}_{\vlambda }\left (\vz ^{(n)}, \cdot \right )}{\pi } &&\quad \text {\textit {Definition of \(d_{\text {TV}}\)}} \nonumber \\ &\quad \leq \sum _{n=1}^N r^{(k-1)\,N + n} &&\quad \text {\textit {\cref {eq:imh_ergodicity}}} \nonumber \\ &\quad = r^{k\,N} \, r^{-N} \, \frac {r - r^{N+1}}{1 - r} \nonumber \\ &\quad = \frac {r \, \left (1 - r^N\right )}{r^N \left (1 - r\right )} \, {\left ( r^{N} \right )}^k. \nonumber \end {alignat} Although the constant depends on \(r\) and \(N\), the kernel \(P\) is geometrically ergodic and converges \(N\) times faster than the base kernel \(K\). \par \paragraph {\textbf {Bound on the Gradient Variance}} To analyze the variance of the gradient, we require detailed information about the \(n\)-step marginal transition kernel, which is unavailable for most MCMC kernels. Fortunately, specifically for the IMH kernel,~\citet {Smith96exacttransition} have shown that the \(n\)-step marginal IMH kernel is given as~\cref {eq:imh_exact_kernel}. \par Furthermore, by \cref {thm:second_moment_bound}, the second moment of the gradient is bounded as \begin {alignat}{2} \E { {\lVert \rvvg _{t,\text {JSA}} \rVert }_2^2 \,\middle |\, \mathcal {F}_{t-1} } &= \V {\rvvg _{t,\text {JSA}} \mid \mathcal {F}_{t-1}} + {\mathsf {Bias}\left [\rvvg _{t,\text {JSA}} \mid \mathcal {F}_{t-1}\right ]}^2 + 2\, \mathsf {Bias}\left [\rvvg _{t,\text {JSA}} \mid \mathcal {F}_{t-1}\right ] \norm {\vmu }_2 + \norm {\vmu }^2_2 \nonumber \\ &\leq \V { \rvvg _{t,\text {JSA}} \mid \mathcal {F}_{t-1}} + {\mathsf {Bias}\left [\rvvg _{t,\text {JSA}} \mid \mathcal {F}_{t-1}\right ]}^2 + 2\,L\,\mathsf {Bias}\left [\rvvg _{t,\text {JSA}} \mid \mathcal {F}_{t-1}\right ] + \norm {\vmu }^2_2, \nonumber \end {alignat} where \(\vmu = \mathbb {E}_{\pi }\vs \left (\vlambda ; \rvvz \right )\). As shown in \cref {thm:mcmc_bias}, the bias terms decreases in a rate of \(r^{t\,N}\). Therefore, \begin {alignat}{2} \E { {\lVert \rvvg _{t,\text {JSA}} \rVert }_2^2 \,\middle |\, \mathcal {F}_{t-1} } &\leq \V { \rvvg _{t,\text {JSA}} \mid \mathcal {F}_{t-1}} + \norm {\vmu }^2_2 + \mathcal {O}\left (r^{t\,N}\right ). &&\quad \text {\textit {\cref {thm:mcmc_bias}}} \nonumber \end {alignat} Note that it is possible to obtain a tighter bound on the bias terms such that \(\mathcal {O}\left (r^{t\,N}/N\right )\), if we directly use \(\left (K, \rvvz \right )\) to bound the bias instead of the higher-level \(\left (P, \rvveta \right )\) abstraction. The extra looseness comes from the use of \cref {thm:product_measure_bound}. \par For the variance term, we show that \begin {alignat}{2} &\V { \rvvg _{t,\mathrm {JSA}} \,\middle |\, \mathcal {F}_{t-1} } \nonumber \\ &\;= \V {\frac {1}{N}\,\sum ^{N}_{n=1}\vs \left (\vlambda ; \rvvz ^{(n)}_t\right ) \,\middle |\, \mathcal {F}_{t-1} } \nonumber \\ &\;= \frac {1}{N^2}\, \sum ^{N}_{n=1} \V { \vs \left (\vlambda ; \rvvz ^{(n)}_t\right ) \,\middle |\, \mathcal {F}_{t-1} } + \frac {2}{N^2} \sum ^{N}_{n=2} \sum ^{n-1}_{m=1} \Cov { \vs \left (\vlambda ; \rvvz ^{(n)}_t\right ), \vs \left (\vlambda ; \rvvz ^{(m)}_t\right ) \,\middle |\, \mathcal {F}_{t-1} } \nonumber \\ &\;\leq \frac {1}{N^2}\sum ^{N}_{n=1} \E { \norm { \vs \left (\vlambda ; \rvvz ^{(n)}_t\right ) }^2_2 \,\middle |\, \mathcal {F}_{t-1} } + C_{\text {cov}} \nonumber \\ &\;= \frac {1}{N^2}\sum ^{N}_{n=1} \E { \norm { \vs \left (\vlambda ; \rvvz ^{(n)}_t\right ) }^2_2 \,\middle |\, \rvvz _{t-1}^{(N)},\, \rvvlambda _{t-1} } + C_{\text {cov}} \nonumber \\ &\;= \frac {1}{N^2}\sum ^{N}_{n=1} \Esub {\rvvz ^{(n)}_t \sim K^n_{\rvvlambda _{t-1}}\left (\vz _{t-1}, \cdot \right )}{ \norm {\vs \left (\vlambda ; \rvvz ^{(n)}_t\right ) }^2_2 \,\middle |\, \rvvz _{t-1}^{(N)},\, \rvvlambda _{t-1} } + C_{\text {cov}} \nonumber \\ &\;\leq \frac {1}{N^2}\sum ^{N}_{n=1} \left [\, n \, {r}^{n-1} \Esub {\rvvz \sim q_{\text {def.}}\left (\cdot ; \rvvlambda _{t-1}\right )}{ \norm {\vs \left (\vlambda ; \rvvz \right )}^2_2 } + {r}^{n} \, \norm {\vs \left (\vlambda ; \rvvz _{t-1}^{(N)} \right )}^2_2 \,\right ] + C_{\text {cov}} &&\quad \text {\textit {\cref {thm:imh_expecation}}} \nonumber \\ &\;\leq \frac {1}{N^2}\sum ^{N}_{n=1} \left [\, n \, {r}^{n-1} \, L^2 + {r}^{n} \, L^2 \,\right ] + C_{\text {cov}} &&\quad \text {\textit {\cref {thm:bounded_score}}} \nonumber \\ &\;= \frac {L^2}{N^2}\sum ^{N}_{n=1} \left [\, n \, {\left (1 - \frac {1}{w^*}\right )}^{n-1} + {\left (1 - \frac {1}{w^*}\right )}^{n} \,\right ] + C_{\text {cov}} \nonumber \\ &\;= \frac {L^2}{N^2} \, \left [\, {\left (w^*\right )}^2 + w^* - {\left (1 - \frac {1}{w^*}\right )}^N \left ( {\left (w^*\right )}^2 + w^* + N\,w^* \right ) \,\right ] + C_{\text {cov}} \nonumber \\ &\;= \frac {L^2}{N^2} \, \left [\, \frac {1}{2} N^2 + \frac {3}{2}\,N + \mathcal {O}\left (1/w^*\right ) \,\right ] + C_{\text {cov}} \nonumber &&\quad \text {\textit {Laurent series expansion at \(w^* \rightarrow \infty \)}} \\ &\;= L^2 \, \left [\, \frac {1}{2} + \frac {3}{2}\,\frac {1}{N} + \mathcal {O}\left (1/w^*\right ) \,\right ] + C_{\text {cov}}, \nonumber \end {alignat} where \[ C_\text {cov} = {\frac {2}{N^2} \sum ^{N}_{n=2} \sum ^{n-1}_{m = 1} \Cov {\vs \left (\vlambda ; \rvvz ^{(n)}_t\right ), \vs \left (\vlambda ; \rvvz ^{(m)}_t\right ) \,\middle |\, \rvvz _{t-1}^{(N)},\, \rvvlambda _{t-1} }}.\] The Laurent approximation becomes exact as \(w^* \rightarrow \infty \), which is useful considering \cref {thm:wstar}.\end{proof}

\prAtEndRestatexiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxiv}\par Our proposed scheme, pMCSA, is described in~\cref {alg:jsa}. At each iteration, our scheme performs a single MCMC transition for each of the \(N\) samples, or chains, to estimate the gradient. That is, \begin {align*} \rvvz ^{(1)}_{t} &\mid \rvvz _{t-1}^{(1)},\, \rvvlambda _{t-1} \sim K_{\rvvlambda _{t-1}}\left (\rvvz _{t-1}^{(1)}, \cdot \right ) \\ \rvvz ^{(2)}_{t} &\mid \rvvz _{t-1}^{(2)},\, \rvvlambda _{t-1} \sim K_{\rvvlambda _{t-1}}\left (\rvvz _{t-1}^{(2)}, \cdot \right ) \\ &\qquad \qquad \vdots \\ \rvvz ^{(N)}_{t} &\mid \rvvz ^{(N)}_{t-1},\, \rvvlambda _{t-1} \sim K_{\rvvlambda _{t-1}}\left (\rvvz _{t-1}^{(N)}, \cdot \right ) \\ \rvvg _{t,\text {pMCSA}} &= -\frac {1}{N}\,\sum ^{N}_{n=1} \, \vs \left (\vlambda , \rvvz ^{(n)}_t\right ), \end {align*} where \(K_{\rvvlambda _{t-1}}^n\) is an \(n\)-transition IMH kernel using \(q_{\text {def.}}\left (\cdot ; \rvvlambda _{t-1}\right )\). \par \paragraph {Ergodicity of the Markov Chain} Since our kernel operates the same MCMC kernel \(K_{\vlambda }\) for each of the \(N\) parallel Markov chains, the \(n\)-step marginal kernel \(P_{\vlambda }\) can be represented as \begin {align*} P_{\vlambda }^k\left (\veta , d\veta ^{\prime }\right ) = K_{\vlambda }^k\left (\vz ^{(1)}, d\vz ^{\prime \; (1)}\right ) \, K_{\vlambda }^k\left (\vz ^{(2)}, d\vz ^{\prime \; (2)}\right ) \cdot \ldots \cdot K_{\vlambda }^k\left (\vz ^{(N)}, d\vz ^{\prime \; (N)}\right ). \end {align*} Then, the convergence in total variation \(d_{\mathrm {TV}}\left (\cdot , \cdot \right )\) can be shown to decrease geometrically as \begin {alignat}{2} &\DTV {K^{k}_{\vlambda }\left (\veta , \cdot \right )}{\Pi } \nonumber \\ &\quad = \sup _{A} \abs { \Pi \left (A\right ) - P^{k}_{\vlambda }\left (\veta , A\right ) } &&\quad \text {\textit {Definition of \(d_{\text {TV}}\)}} \nonumber \\ &\quad \leq \sup _{A} \big |\; \int _{A} \pi \left (d\vz ^{\prime }_1\right ) \cdot \ldots \cdot \pi \left (d\vz ^{\prime }_N\right ) \nonumber \\ &\qquad \qquad \qquad - K^k_{\vlambda }\left (\vz _1, d\vz ^{\prime }_1\right ) \cdot \ldots \cdot K^k_{\vlambda }\left (\vz _N, d\vz ^{\prime }_N\right ) \;\big | \nonumber \\ &\quad \leq \sup _{A} \sum _{n=1}^N \abs { \int _{A} \pi \left (d\vz ^{\prime }_k\right ) - K^{k}_{\vlambda }\left (\vz _n, d\vz ^{\prime }_n\right ) } &&\quad \text {\textit {\cref {thm:product_measure_bound}}} \nonumber \\ &\quad = \sum _{n=1}^N \DTV {K^k_{\vlambda }\left (\vz _n, \cdot \right )}{\pi } &&\quad \text {\textit {\cref {eq:imh_ergodicity}}} \nonumber \\ &\quad \leq \sum _{n=1}^N r^{k} &&\quad \text {\textit {Geometric ergodicity}} \nonumber \\ &\quad = N\,r^{k}. \nonumber \end {alignat} \par \paragraph {\textbf {Bound on the Gradient Variance}} By \cref {thm:second_moment_bound}, the second moment of the gradient is bounded as \begin {alignat}{2} \E { {\lVert \rvvg _{t,\text {pMCSA}} \rVert }_2^2 \,\middle |\, \mathcal {F}_{t-1} } &= \V {\rvvg _{t,\text {pMCSA}} \mid \mathcal {F}_{t-1}} + {\mathsf {Bias}\left [\rvvg _{t,\text {pMCSA}} \mid \mathcal {F}_{t-1}\right ]}^2 + 2\, \mathsf {Bias}\left [\rvvg _{t,\text {pMCSA}} \mid \mathcal {F}_{t-1}\right ] \norm {\vmu }_2 + \norm {\vmu }^2_2 \nonumber \\ &\leq \V { \rvvg _{t,\text {pMCSA}} \mid \mathcal {F}_{t-1}} + {\mathsf {Bias}\left [\rvvg _{t,\text {pMCSA}} \mid \mathcal {F}_{t-1}\right ]}^2 + 2\,L\,\mathsf {Bias}\left [\rvvg _{t,\text {pMCSA}} \mid \mathcal {F}_{t-1}\right ] + \norm {\vmu }^2_2, \nonumber \end {alignat} where \(\vmu = \mathbb {E}_{\pi }\vs \left (\vlambda ; \rvvz \right )\). As shown in \cref {thm:mcmc_bias}, the bias terms decreases in a rate of \(r^{t}\). Therefore, \begin {alignat}{2} \E { {\lVert \rvvg _{t,\text {pMCSA}} \rVert }_2^2 \,\middle |\, \mathcal {F}_{t-1} } &\leq \V { \rvvg _{t,\text {pMCSA}} \mid \mathcal {F}_{t-1}} + \norm {\vmu }^2_2 + \mathcal {O}\left (r^{t}\right ). &&\quad \text {\textit {\cref {thm:mcmc_bias}}} \nonumber \end {alignat} As noted in the proof of \cref {thm:jsa}, it is possible to obtain a tighter bound on the bias terms such that \(\mathcal {O}\left (r^{t}/N\right )\). \par The variance term is bounded as \begin {alignat}{2} &\V { \rvvg _{t,\text {pMCSA}} \mid \mathcal {F}_{t-1}} \nonumber \\ &\quad = \V { \frac {1}{N}\sum ^{N}_{n=1} \vs \left (\vlambda ; \rvvz ^{(n)}_t\right ) \,\middle |\, \rvvz _{t-1}^{(1:N)},\, \rvvlambda _{t-1} } \nonumber \\ &\quad = \frac {1}{N^2}\sum ^{N}_{n=1} \V { \vs \left (\vlambda ; \rvvz ^{(n)}_t\right ) \,\middle |\, \rvvz _{t-1}^{(1:N)},\, \rvvlambda _{t-1} } &&\quad \text {\textit {\(\rvvz ^{(i)}_t \,\bot \, \rvvz ^{(j)}_t\) for \(i \neq j\)}} \nonumber \\ &\quad \leq \frac {1}{N^2}\sum ^{N}_{n=1} \E { \norm {\vs \left (\vlambda ; \rvvz ^{(n)}_t\right ) }^2_2 \,\middle |\, \rvvz _{t-1}^{(1:N)},\, \rvvlambda _{t-1} }_2 \nonumber \\ &\quad = \frac {1}{N^2}\sum ^{N}_{n=1} \Esub {\rvvz ^{(n)}_t \sim K_{\rvvlambda _{t-1}}\left (\rvvz _{t-1}^{(n)}, \cdot \right )}{ \norm {\vs \left (\vlambda ; \rvvz ^{(n)}_t\right ) }^2_2 \,\middle |\, \rvvz _{t-1}^{(1:N)},\, \rvvlambda _{t-1} } \nonumber \\ &\quad \leq \frac {1}{N^2}\sum ^{N}_{n=1} \left [\, \Esub {\rvvz \sim q_{\text {def.}}\left (\cdot ;\rvvlambda _{t-1}\right )}{ \norm {\vs \left (\vlambda ; \rvvz \right )}^2_2 } + {r} \, \norm {\vs \left (\vlambda ; \rvvz _{t-1}^{(n)} \right )}^2_2 \,\right ] &&\quad \text {\textit {\cref {thm:imh_expecation}}} \nonumber \\ &\quad \leq \frac {1}{N^2}\sum ^{N}_{n=1} \left [\, L^2 + {r} \, L^2 \,\right ] &&\quad \text {\textit {\cref {thm:bounded_score}}} \nonumber \\ &\quad = \frac {L^2}{N^2} \sum ^{N}_{n=1} \left [\, 1 + {r} \,\right ] \nonumber \\ &\quad = L^2 \left [\, \frac {1}{N} + \frac {1}{N}\,{\left (1 - \frac {1}{w^*}\right )} \,\right ]. \nonumber \end {alignat}\end{proof}


==> paretok_additional.tex <==

\subsection{Additional Results of Logistic Regression Experiments}


\begin{figure}[H]
  \centering
  \subfloat[Pima]{
    \includegraphics[scale=0.80]{figures/pima_01.pdf}
  }
  \subfloat[Heart]{
    \includegraphics[scale=0.80]{figures/heart_01.pdf}
  }
  \caption{Pareto-\(\widehat{k}\) results of logistic regression problems.
    The solid lines are the median of 100 repetitions while the colored regions are the 80\% empirical percentiles.
  }
\end{figure}

%%% Local Variables:
%%% TeX-master: "master"
%%% End:


==> pimh_algorithm.tex <==

\hspace{0.04\textwidth}
\begin{minipage}[r]{0.45\textwidth}
  \small
  \begin{algorithm2e}[H]
    \DontPrintSemicolon
    \SetAlgoLined
    \KwIn{initial samples \(\vz_0^{(1)},\, \ldots,\, \vz_0^{(N)}\),
      initial parameter \(\vlambda_0\),
      number of iterations \(T\),
      stepsize schedule \(\gamma_t\)
    }
    \For{\textcolor{black}{\(t = 1, 2, \ldots, T\)}}{
      \textcolor{blue}{
        \For{\textcolor{blue}{\(i = 1, 2, \ldots, N\)}}{
          \(\vz^{(i)}_{t} \sim K(\vz^{(i)}_{t-1}, \cdot)\)\;
        }
      }
      \( s(\vz^{(i)}_t; \vlambda) = \nabla_{\vlambda} \log q_{\vlambda}(\vz_t^{(i)}) \)\;
      \( \vlambda_{t} = \vlambda_{t-1} + \gamma_t\,
      \textcolor{purple}{\frac{1}{N} \sum^{N}_{i=1} s\,(\vz_t^{(i)};\vlambda_{t-1})} \)\;
    }
    \caption{Markovian Score Climbing with Parallel Chains}\label{alg:pimh}
  \end{algorithm2e}
\end{minipage}
\hspace{0.02\textwidth}
\begin{minipage}[l]{0.37\textwidth}
  \small
  \begin{algorithm2e}[H]
    \DontPrintSemicolon
    \SetAlgoLined
    \KwIn{previous sample \(\vz_{t-1}\),
      previous parameter \(\vlambda_{t-1}\),
    }
    \(\vz^* \sim q_{\vlambda_{t-1}}(\vz)\)\;
    \(w(\vz) = p(\vz,\vx)/q_{\vlambda_{t-1}}(\vz) \)\;
    \(\alpha = \min\left( w\,(\vz^*)/w\,(\vz_{t-1}), 1\right)\)\;
    \(u \sim \mathrm{Uniform}(0, 1) \)\;
    \eIf{u < \(\alpha\)}
        {
          %\(\vz_t \leftarrow \vz^*\)
          \(\vz_t = \vz^*\)
        }
        {
          %\(\vz_t \leftarrow \vz_{t-1}\)
          \(\vz_t = \vz_{t-1}\)
        }
        \caption{\\ Independent Metropolis-Hastings}\label{alg:imh}
  \end{algorithm2e}
\end{minipage}
\hspace{0.04\textwidth}

%%% Local Variables:
%%% TeX-master: "master"
%%% End:


==> pratenddefaultcategory.tex <==

\prAtEndRestateii*
\label{proofsection:prAtEndii}\begin{proof}[Proof of \autoref{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}For notational convenience, we define the shorthand \begin {align*} \pi \left (\vz _{(1:N)}\right ) = \pi \left (\vz _1\right ) \, \pi \left (\vz _2\right ) \times \ldots \times \pi \left (\vz _N\right ). \end {align*} Then, \begin {alignat}{2} &\Esub {\Pi }{ f\left (\vlambda , \veta \right ) } \nonumber \\ &\quad = \int \left ( \frac {1}{N} \sum ^{N}_{n=1} \log q\left (\vz _n; \vlambda \right ) + \mathbb {H}\left [\,\pi \,\right ]\right ) \, \pi \left (\vz _{(1:N)}\right ) \, d\vz _{(1:N)} \nonumber \\ &\quad = \frac {1}{N} \sum ^{N}_{n=1} \left \{ \int \big (\, \log q\,(\,\vz _n; \vlambda \,) + \mathbb {H}\,[\,\pi \,] \,\big ) \, \pi \left (\vz _{(1:N)}\right ) \, d\vz _{(1:N)} \right \} &&\quad {\text {\textit {Swapped integral and sum}}} \nonumber \\ &\quad = \frac {1}{N} \sum ^{N}_{n=1} \int \big (\, \log q\,(\,\vz _n; \vlambda \,) + \mathbb {H}\,[\,\pi \,] \,\big ) \, \pi \left (\vz _n\right ) \, d\vz _{n} &&\quad {\text {\textit {Marginalized \(\vz _m\) for all \(m \neq n\)}}} \nonumber \\ &\quad = \frac {1}{N} \sum ^{N}_{n=1} \DKL {\pi }{q\left (\cdot ; \vlambda \right )} \nonumber &&\quad {\text {\textit {Definition of \(D_{\text {KL}}\)}}} \\ &\quad = \DKL {\pi }{q\left (\cdot ; \vlambda \right )}\label {eq:F_KL} \end {alignat} For \(\Esub {\Pi }{ g\left (\vlambda , \rvveta \right ) }\), note that \begin {align} \nabla _{\vlambda } f\left (\vlambda , \veta \right ) = \frac {1}{N} \sum ^{N}_{n=1} s\left (\vz _n; \vlambda \right ) = g\left (\vlambda , \veta \right ).\label {eq:F_grad_G} \end {align} Therefore, it suffices to show that \begin {align*} \nabla _{\vlambda } \DKL {\pi }{q\left (\cdot ; \vlambda \right )} &= \nabla _{\vlambda } \Esub {\Pi }{ f\left (\vlambda , \rvveta \right ) } &&\text {\textit {\cref {eq:F_KL}}} \\ &= \Esub {\Pi }{ \nabla _{\vlambda } f\left (\vlambda , \rvveta \right ) } &&\text {\textit {{Leibniz derivative rule}}} \\ &= \Esub {\Pi }{ g\left (\vlambda , \rvveta \right ) }. &&\text {\textit {\cref {eq:F_grad_G}}} \end {align*}\end{proof}
\begin{restatable}[]{lemma}{prAtEndRestateiii}\label{thm:prAtEndiii}\label {thm:additive} The bivariate function location and scale reparameterization function \( t\left (\vu , \vlambda \right ) = \mC \,\vu + \vm \) is additive with respect to \(\vlambda =\left [\mC , \vm \right ]\) such that \[ t\left (\vu , \alpha \,\vlambda + \beta \,\vmu \right ) = \alpha \,t\left (\vu , \vlambda \right ) + \beta \,t\left (\vu , \vmu \right ) \] for any \(\alpha \), \(\beta \).\end{restatable}
\label{proofsection:prAtEndiii}\begin{proof}[Proof of \autoref{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}Let us denote \(\vlambda =\left [\mC _{\vlambda }, \vm _{\vlambda }\right ]\) and \(\vmu = \left [\mC _{\vmu }, \vm _{\vmu }\right ]\). Then, \begin {alignat}{2} t\left (\vu , \alpha \,\vlambda + \beta \,\vmu \right ) &= \left (\alpha \,\mC _{\vlambda } + \beta \,\mC _{\vmu }\right )\,\vu + \left (\alpha \,\vm _{\vlambda } + \beta \,\vm _{\vmu }\right ) \nonumber \\ &= \alpha \,\left (\mC _{\vlambda }\vu + \vm _{\vlambda }\right ) + \beta \,\left (\mC _{\vmu }\,\vu + \vm _{\vmu }\right ) \nonumber \\ &= \alpha \,t\left (\vu , \vlambda \right ) + \beta \,t\left (\vu , \vmu \right ). \nonumber \end {alignat}\end{proof}
\prAtEndRestateiv*
\label{proofsection:prAtEndiv}\begin{proof}[Proof of \autoref{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}A distribution \(q\left (\cdot \right ) \in \mathcal {Q}\) in a location-scale family \(\mathcal {Q}\) is defined as \begin {align*} \rvvz \sim q\left (\cdot \right ) \iff \rvvz = t\left (\rvvu , \vlambda \right ),\; \rvvu \sim \phi \left (\cdot \right ). \end {align*} The reparameterization function \(t\) is defined as an affine transformation \begin {align*} t\left (\vu , \vlambda \right ) = \mC \,\vu + \vm \end {align*} for the location \(\vm \) and scale \(\mC \) parameters and their concatenation \(\vlambda = \left [\mC , \vm \right ]\). \par Furthermore, the base density \(\phi \left (\vz \right )\) of any location-scale log-concave family is log-concave. Therefore, it follows that \begin {alignat}{2} &\log \phi \left (t\left (\vu , \alpha \vlambda + (1 - \alpha )\,\vmu \right )\right ) \nonumber \\ &\quad = \log \phi \left ( \alpha \,t\left (\vu , \vlambda \right ) + (1 - \alpha )\,t\left (\vu , \vmu \right )\right ) &&\quad \text {\textit {\cref {thm:additive}}} \nonumber \\ &\quad = \alpha \,\log \phi \left (t\left (\vu , \vlambda \right )\right ) + (1 - \alpha )\,\log \phi \left (t\left (\vu , \vmu \right )\right ) &&\quad \text {\textit {Log-concavity of \(\phi \)}}. \nonumber \end {alignat}\end{proof}
\begin{restatable}[]{lemma}{prAtEndRestatev}\label{thm:prAtEndv}\label {thm:mixing_time} Assuming the kernel \(P_{\vlambda }\left (\veta , \cdot \right )\) satisfies \cref {thm:ergodicity}, the Hellinger mixing time \(\tau _{\text {Hel.}}\) is bounded as \begin {align*} \tau _{\text {Hel.}}\left (K_{\vlambda }, \epsilon \right ) \leq \frac {2}{\log \rho ^{-1}} \log \frac {1}{\epsilon } \end {align*}\end{restatable}
\label{proofsection:prAtEndv}\begin{proof}[Proof of \autoref{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}The following two inequalities are equivalent. \begin {align*} d_{\text {Hel.}}\left (\, P^t_{\vlambda }\left (\veta , \cdot \right ), \Pi \,\right ) &\leq \sqrt {\DTV { P^t_{\vlambda }\left (\veta , \cdot \right )}{\Pi }} \leq \rho ^{t / 2} \\ \log d_{\text {Hel.}}\left (\, P^t_{\vlambda }\left (\veta , \cdot \right ), \Pi \,\right ) &\leq \frac {t}{2} \log \rho \end {align*} \par The Hellinger mixing time \(\tau _{\text {Hel.}}\left (K_{\vlambda }, \epsilon \right )\) is the smallest \(t\) that statisfies the inequality \begin {align*} d_{\text {Hel.}}\left (\, P^t_{\vlambda }\left (\veta , \cdot \right ), \Pi \,\right ) &\leq \epsilon . \end {align*} Instead, we can find the \(t\prime > t\) that satisfies \begin {align*} \log d_{\text {Hel.}}\left (\, P^t_{\vlambda }\left (\veta , \cdot \right ), \Pi \,\right ) \leq \frac {t\prime }{2} \log \rho \leq \log \epsilon \end {align*} by solving the inequalities \begin {alignat*}{2} \frac {t\prime }{2} \log \rho &\leq \log \epsilon \\ t\prime &\geq \frac {2}{\log \rho } \log \epsilon &&\quad \text {\textit {Inequality flipped since \(\log \rho \leq 1\)}} \\ t\prime &\geq \frac {2}{\log \rho ^{-1}} \log \frac {1}{\epsilon } \end {alignat*}\end{proof}
\prAtEndRestatevi*
\label{proofsection:prAtEndvi}\begin{proof}[Proof of \autoref{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}\citet [Corollary 3.5]{duchi_ergodic_2012} provide a non-asymptotic convergence rate for the \textit {ergodic mirror descent} algorithm which computes the parameter update as \begin {align} \vlambda _{t+1} &= \argmin _{\vlambda \in \Lambda } \left \{\, \iprod {\,\vg \left (\vlambda , \veta _t\right )}{\vlambda \,} + \frac {1}{\alpha _t} D_{\psi }\left (\vlambda , \vlambda _{t}\right ) \,\right \}\label {eq:ergodic_mirror_descent} \\ \rvveta _{t+1} &\sim P_{\vlambda _{t}}\left (\veta _t, \cdot \right ) \nonumber \end {align} where \(D_{\psi }\) is the Bregman divergence defined as \begin {align*} D_{\psi }\left (\vlambda , \vlambda \prime \right ) \triangleq \psi \left (\vlambda \right ) - \psi \left (\vlambda \prime \right ) - \iprod { \nabla \psi \left (\vlambda \prime \right )}{\vlambda - \vlambda \prime } \end {align*} for some convex function \(\psi \). Our result is based on the fact that MCGD is a special case of the ergodic mirror descent algorithm. Specifically, by choosing \(\psi \left (\vlambda \right ) = \frac {1}{2} \norm {\vlambda }^2_2 \), we obtain \begin {alignat}{2} D_{\psi }\left (\vlambda , \vlambda \prime \right ) = \frac {1}{2} \norm {\vlambda - \vlambda \prime }_2^2 \leq \frac {1}{2} \, R^2.\label {eq:bregman} &&\quad \text {\textit {\cref {thm:compact}}} \end {alignat} This reduces the update in \cref {eq:ergodic_mirror_descent} into projected gradient descent which is the form used for Markov chain score climbing. \par Under our assumptions, \citet [Corollary 3.5]{duchi_ergodic_2012} show that, by assuming that the Hellinger mixing time is bounded as \begin {align} \tau _{\text {Hel.}}\left (K_{\vlambda }, \epsilon \right ) \leq \kappa _1 \log \left ( \kappa _2 /\epsilon \right ) \label {eq:hellinger_mixing} \end {align} for any \(\epsilon > 0\), and setting a decreasing stepsize \(\alpha _t = \alpha / \sqrt {t}\), it follows that \begin {align} &\E { \DKL {\pi }{q\,(\cdot ; {\overline {\vlambda }_{T}})} - \DKL {\pi }{q\left (\cdot ; {\vlambda ^*}_{T}\right )}} \nonumber \\ &\quad \leq \frac {R^2}{2 \, \alpha \, \sqrt {T}} + \frac {2 \, \alpha \, G^2}{\sqrt {T}}\left ( \kappa _1 \, \log \frac {\kappa _2}{\epsilon } \right ) + 3 \, \epsilon \, G \, R + \frac {R \, G \, \kappa _1 \, \log \frac {\kappa _2}{\epsilon }}{T}.\label {eq:original_bound} \end {align} \par From this, by setting the initial stepsize as \(\alpha = R / \left (G \sqrt {\kappa _1 \log \left (\kappa _2 \, T\right ) }\right )\) and \(\epsilon = 1/ \sqrt {T}\), \begin {alignat*}{2} &\E { \DKL {q\,(\cdot ; {\overline {\vlambda }_{T}})}{\pi } - \DKL {q\left (\cdot ; {\vlambda ^*}_{T}\right )}{\pi }} \\ &\leq \frac {R}{2 \, \alpha \, \sqrt {T}} + \frac {2 \, \alpha \, G^2}{\sqrt {T}}\left ( \kappa _1 \, \log \frac {\kappa _2}{\epsilon } \right ) + 3 \, \epsilon \, G \, R + \frac {R \, G \, \kappa _1 \, \log \frac {\kappa _2}{\epsilon }}{T}. &&\quad \text {\textit {\cref {eq:original_bound}}} \\ &= \frac {R \, G \, \sqrt {\kappa _1 \, \log \left (\kappa _2 \, T\right ) } }{2 \, \sqrt {T}} + \frac {2 \, R \, G}{\sqrt {T}} \frac { \kappa _1 \, \log \kappa _2 \, \sqrt {T} }{ \sqrt {\kappa _1 \log \left (\kappa _2 \, T\right )}} + \frac {3 \, G \, R}{\sqrt {T}} + \frac {R \, G \, \kappa _1 \, \log \left (\kappa _2 \, \sqrt {T}\right )}{T} &&\quad \text {\textit {Plugged value of \(\epsilon \) and \(\alpha \)}} \\ &\leq \frac {R \, G \, \sqrt {\kappa _1 \, \log \left (\kappa _2 \, T\right ) } }{2 \, \sqrt {T}} + \frac {2 \, R \, G}{\sqrt {T}} \frac { \kappa _1 \, \log \kappa _2 \, T }{ \sqrt {\kappa _1 \log \left (\kappa _2 \, T\right )}} + \frac {3 \, G \, R}{\sqrt {T}} + \frac {R \, G \, \kappa _1 \, \log \left (\kappa _2 \, T\right )}{T} &&\quad \text {\textit {Applied \(\log \sqrt {T} < \log T\)}} \\ &= \frac {R \, G \, \sqrt {\kappa _1 \, \log \left (\kappa _2 \, T\right ) } }{2 \, \sqrt {T}} + \frac {2 \, R \, G}{\sqrt {T}} \sqrt {\kappa _1 \, \log \left ( \kappa _2 \, T\right ) } + \frac {3 \, G \, R}{\sqrt {T}} + \frac {R \, G \, \kappa _1 \, \log \left (\kappa _2 \, T\right )}{T} &&\quad \text {\textit {Solved fraction}} \\ &= \frac {5 \, R \, G \, \sqrt {\kappa _1 \, \log \left (\kappa _2 \, T\right ) } }{2 \, \sqrt {T}} + \frac {3 \, G \, R}{\sqrt {T}} + \frac {R \, G \, \kappa _1 \, \log \left (\kappa _2 \, T\right )}{T}. &&\quad \text {\textit {Combined fractions}} \end {alignat*} \par From \cref {thm:mixing_time}, we retrieve the constants of \cref {eq:hellinger_mixing} as \( \kappa _1=\frac {2}{\log \rho ^{-1} },\; \kappa _2 = 1 \), which follows our result \begin {alignat*}{2} &\frac { 5 \, R \, G \, \sqrt {\kappa _1 \, \log \left (\kappa _2 \, T\right ) } }{ 2 \, \sqrt {T} } + \frac {3 \, G \, R}{\sqrt {T}} + \frac {R \, G \, \kappa _1 \, \log \left (\kappa _2 \, T\right )}{T} \\ &\quad = \frac { 5 \, R \, G \, \sqrt { \frac {2}{\log \rho ^{-1}} \, \log T } }{ 2 \, \sqrt {T} } + \frac {3 \, G \, R}{\sqrt {T}} + \frac {R \, G \, \frac {2}{\log \rho ^{-1}} \, \log T}{T} &&\quad \text {\textit {Plugged values of \(\kappa _1\) and \(\kappa _2\)}} \\ &\quad = \frac { 5 \, \sqrt {2} \, R \, }{ 2 } \, \frac { G \, \sqrt {\log T} }{ \log \rho ^{-1} \, \sqrt {T} \, } + 3 \, R \, \frac {G \, R}{\sqrt {T}} + 2 \, R \, \frac {G \, \log T}{ \log \rho ^{-1} \, T} &&\quad \text {\textit {Pulled constants forward}} \end {alignat*}\end{proof}
\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {thm:product_measure_bound} For the probability measures \(p_1, \ldots , p_N\) and \(q_1, \ldots , q_N\) defined on a measurable space \((\mathsf {X}, \mathcal {A})\) and an arbitrary set \(A \in \mathcal {A}\), \begin {align*} &\abs { \int _{A^N} p_1\left (dx_1\right ) p_2\left (dx_2\right ) \times \ldots \times p_N\left (dx_N\right ) - q_1\left (dx_1\right ) q_2\left (dx_2\right ) \times \ldots \times q_N\left (dx_N\right ) } \\ &\qquad \leq \sum _{n=1}^N \abs { \int _{A} p_n\left (dx_n\right ) - q_n\left (dx_n\right ) } \end {align*}\end{restatable}
\label{proofsection:prAtEndvii}\begin{proof}[Proof of \autoref{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}By using the following shorthand notations \begin {alignat*}{2} p_{(1:N)}\left (dx_{(1:N)}\right ) &= p_1\left (dx_1\right ) p_2\left (dx_2\right ) \times \ldots \times p_N\left (dx_N\right ) \\ q_{(1:N)}\left (dx_{(1:N)}\right ) &= q_1\left (dx_1\right ) q_2\left (dx_2\right ) \times \ldots \times q_N\left (dx_N\right ), \end {alignat*} the result follows from induction as \begin {alignat}{2} &\abs { \int _{A^N} p_{(1:N)}\left (dx_{(1:N)}\right ) - q_{(1:N)}\left (dx_{(1:N)}\right ) } \nonumber \\ &\quad = \Bigg |\; \left ( \int _{A} p_1\left (dx_1\right ) - q_1\left (dx_1\right ) \right ) \, \int _{A^{N-1}} p_{(2:N)}\left (dx_{(2:N)}\right ) \nonumber \\ &\qquad \quad + \int _{A} q_1\left (dx_1\right ) \, {\left ( \int _{A^{N-1}} p_{(2:N)}\left (dx_{(2:N)}\right ) - q_{(2:N)}\left (dx_{(2:N)}\right ) \right )} \;\Bigg | \nonumber \\ &\quad \leq \Bigg | \int _{A} p_1\left (dx_1\right ) - q_1\left (dx_1\right ) \Bigg |\; \int _{A^{N-1}} p_{(2:N)}\left (dx_{(2:N)}\right ) \nonumber \\ &\qquad \quad + \int _{A} q_1\left (dx_1\right ) \, { \Bigg |\; \int _{A^{N-1}} p_{(2:N)}\left (dx_{(2:N)}\right ) - q_{(2:N)}\left (dx_{(2:N)}\right ) } \;\Bigg | &&\quad \text {\textit {Triangle inequality}} \nonumber \\ &\quad \leq \Bigg | \int _{A} p_1\left (dx_1\right ) - q_1\left (dx_1\right ) \Bigg |\; \nonumber \\ &\qquad \quad + { \Bigg |\; \int _{A^{N-1}} p_{(2:N)}\left (dx_{(2:N)}\right ) - q_{(2:N)}\left (dx_{(2:N)}\right ) } \;\Bigg |. &&\quad \text {\textit {Applied \(p_n\left (A\right ), q_n\left (A\right ) \leq 1 \)}} \nonumber \end {alignat}\end{proof}
\prAtEndRestateviii*
\label{proofsection:prAtEndviii}\begin{proof}[Proof of \autoref{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}the ergodic convergence rate of the i-SIR kernel is given by \citet {andrieu_uniform_2018}. \begin {alignat*}{2} \DTV {P^{k}\left (\veta , \cdot \right )}{\Pi } = \DTV {K^{k}\left (\vz , \cdot \right )}{\pi } \leq {\left (1 - \frac {N - 1}{2 w^* + N - 2}\right )}^k \end {alignat*} \par \begin {alignat}{2} &\E { \norm { g\left (\cdot , \rvveta \right ) }^2_{*} \,\middle |\, \mathcal {F}_{t} } \nonumber \\ &\quad = \E { \norm { g\left (\cdot , \rvveta \right ) }^2 \,\middle |\, \vz _{t-1},\, \vlambda _{t-1} } \nonumber \\ &\quad = \Esub {\rvvz \sim K\left (\vz _{t-1}, \cdot \right )}{ \norm { s\left (\cdot ; \rvvz \right ) }^2_{*} \,\middle |\, \vz _{t-1},\, \vlambda _{t-1} } \nonumber \\ &\quad = \int \sum ^{N}_{n=1} \frac { w\left (\vz _n\right ) }{ \sum ^{N}_{m=1} w\left (\vz _m\right ) } \norm { s\left (\cdot ; \vz _n\right ) }^2_{*} \prod ^{N}_{n=2} q\left (d\vz _n; \vlambda _{t-1}\right ) \nonumber \\ &\quad = \int \sum ^{N}_{n=1} \overline {w}\left (\vz _n\right ) \norm { s\left (\cdot ; \vz _n\right ) }^2_{*} \prod ^{N}_{n=2} q\left (d\vz _n\right ) \nonumber &&\quad \text {\textit { Define {\small \( {\overline {w}}\left (\vz _n\right ) = \frac { w\left (\vz _n\right ) }{ \sum ^{N}_{m=1} w\left (\vz _m\right ) } \) }}} \\ &\quad = \int \left ( \vw ^{\top }\, \vf \, \right ) \prod ^{N}_{n=2} q\left (d\vz _n; \vlambda _{t-1}\right ) \nonumber &&\quad \text {\textit { Define vectors {\small \( {\left [\vw \right ]}_n = \overline {w}\left (\vz _n\right ) \) }and {\small \( {\left [\,\vf \,\right ]}_n = \norm { s\left (\cdot ; \vz _n\right ) }^2_{*} \) }}} \\ &\quad \leq \sqrt { \Esub { q\left (\cdot , \vlambda _{t-1}\right ) }{ \vw ^{\top } \vw } \Esub { q\left (\cdot , \vlambda _{t-1}\right ) }{ \,\vf ^{\top }\vf \, } } \nonumber &&\quad \text {\textit {Cauchy-Schwarz inequality}} \\ &\quad = \sqrt { \Esub { \rvvz _n \sim q\left (\cdot , \vlambda _{t-1}\right ) }{ \sum ^{N}_{n=1} {\left ( \overline {w}\left (\rvvz _n\right ) \right )}^2 } \Esub { \rvvz _n \sim q\left (\cdot , \vlambda _{t-1}\right ) }{ \norm { s\left (\cdot ; \vz _n\right ) }^4_{*} } } \nonumber \\ &\quad \leq \sqrt { \Esub { \rvvz _n \sim q\left (\cdot , \vlambda _{t-1}\right ) }{ \norm { s\left (\cdot ; \vz _n\right ) }^4_{*} } } \nonumber &&\quad \text {\textit {Applied \(\sum ^N_{n=1} {\left (\overline {w}\left (\vz _n\right )\right )}^2 \leq \sum ^N_{n=1} \overline {w}\left (\vz _n\right ) = 1\)}} \\ &\quad \leq \sqrt { \sigma ^4 } \nonumber \\ &\quad = \sigma ^2 \nonumber \end {alignat} \par \end{proof}
\begin{restatable}[]{lemma}{prAtEndRestateix}\label{thm:prAtEndix}\label {thm:lambda_bound} For \(w^* = \sup _{\vz } w\left (\vz \right ) \), \(\lambda \left (\cdot \right )\) in~\cref {eq:T_lambda} is bounded as \[ \max \left (1 - \frac {1}{w}, 0\right ) \leq \lambda \left (w\right ) \leq 1 - \frac {1}{w^*}. \]\end{restatable}
\label{proofsection:prAtEndix}\begin{proof}[Proof of \autoref{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}The proof can be found in the proof of Theorem 3 of \citet {Smith96exacttransition}.\end{proof}
\begin{restatable}[]{lemma}{prAtEndRestatex}\label{thm:prAtEndx}\label {thm:tn_bound} For \(w^* = \sup _{\vz } w\left (\vz \right ) \), \(T_t\left (\cdot \right )\) in~\cref {eq:T_lambda} is bounded as \[ T_n\left ( w \right ) \leq \frac {n}{w} \, {\left (1 - \frac {1}{w^*}\right )}^{n-1}. \]\end{restatable}
\label{proofsection:prAtEndx}\begin{proof}[Proof of \autoref{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}\begin {alignat*}{2} T_n\left (w\right ) &= \int _w^{\infty } \frac {n}{v^2} \, \lambda ^{n-1}\left (v\right )\,dv &&\quad \text {\textit {\cref {eq:T_lambda}}} \\ &\leq \int _w^{\infty } \frac {n}{v^2} \, {\left (1 - \frac {1}{w^*}\right )}^{n-1}\,dv &&\quad \text {\textit {\cref {thm:lambda_bound}}} \\ &= n \, {\left (1 - \frac {1}{w^*}\right )}^{n-1} \int _w^{\infty } \frac {1}{v^2} \,dv &&\quad \text {\textit {Pulled out constant}} \\ &= n \, {\left (1 - \frac {1}{w^*}\right )}^{n-1} \left ( {-\left .\frac {1}{v}\right \rvert ^{\infty }_{w}} \right ) &&\quad \text {\textit {Solved indefinite integral}} \\ &= \frac {n}{w} \, {\left (1 - \frac {1}{w^*}\right )}^{n-1}. \end {alignat*} This upper bound is in general difficult to improve unless we impose stronger assumptions on \(\pi \) and \(q\).\end{proof}
\begin{restatable}[]{lemma}{prAtEndRestatexi}\label{thm:prAtEndxi}\label {thm:imh_expecation} For a positive test function \(f : \mathcal {Z} \rightarrow \mathbb {R}^{+}\), the estimate of a \(\pi \)-invariant independent Metropolis-Hastings kernel with a proposal \(q\) is bounded as \begin {align*} \Esub {K^n\left (\vz , \cdot \right )}{ f \,\middle |\, \vz } \leq n \, {\left (1 - \frac {1}{w^*}\right )}^{n-1} \Esub {q}{f} + {\left (1 - \frac {1}{w^*}\right )}^n \, f\left (\vz \right ) \end {align*} where \(w\left (\vz \right ) = \pi \left (\vz \right ) / q\left (\vz \right )\) and \(w^* = \sup _{\vz } w\left (\vz \right ) \).\end{restatable}
\label{proofsection:prAtEndxi}\begin{proof}[Proof of \autoref{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}\begin {alignat*}{2} &\Esub {K^n\left (\vz , \cdot \right )}{ f \,\middle |\, \vz } \\ &\quad = \int T_n\left (w\left (\vz \right ) \vee w\left (\vz \prime \right )\right ) \, f\left (\vz \prime \right ) \, \pi \left (\vz \prime \right ) d\vz \prime + \lambda ^{n}\left (w\left (\vz \right )\right ) \, f\left (\vz \right ) &&\quad {\text {\textit {\cref {eq:imh_exact_kernel}}}} \\ &\quad \leq \int \frac {n}{w\left (\vz \right ) \vee w\left (\vz \prime \right )} \, {\left (1 - \frac {1}{w^*}\right )}^{n-1} \, f\left (\vz \prime \right ) \, \pi \left (\vz \prime \right ) d\vz \prime + \lambda ^{n}\left (w\left (\vz \right )\right ) \, f\left (\vz \right ) &&\quad {\text {\textit {\cref {thm:tn_bound}}}} \\ &\quad \leq \int \frac {n}{w\left (\vz \prime \right )} \, {\left (1 - \frac {1}{w^*}\right )}^{n-1} \, f\left (\vz \prime \right ) \, \pi \left (\vz \prime \right ) d\vz \prime + \lambda ^{n}\left (w\left (\vz \right )\right ) \, f\left (\vz \right ) &&\quad {\frac {1}{w\left (\vz \right ) \vee w\left (\vz \prime \right )} \leq \frac {1}{w\left (\vz \prime \right )}} \\ &\quad = n \, {\left (1 - \frac {1}{w^*}\right )}^{n-1} \, \int \frac {1}{w\left (\vz \prime \right )} \, f\left (\vz \prime \right ) \, \pi \left (\vz \prime \right ) d\vz \prime + \lambda ^{n}\left (w\left (\vz \right )\right ) \, f\left (\vz \right ) &&\quad {\text {\textit {Pulled out constant}}} \\ &\quad = n \, {\left (1 - \frac {1}{w^*}\right )}^{n-1} \, \int f\left (\vz \prime \right ) \, q\left (\vz \prime \right ) d\vz \prime + \lambda ^{n}\left (w\left (\vz \right )\right ) \, f\left (\vz \right ) &&\quad {\text {\textit {Definition of \(w\left (\vz \right )\)}}} \\ &\quad \leq n \, {\left (1 - \frac {1}{w^*}\right )}^{n-1} \, \int f\left (\vz \prime \right ) \, q\left (\vz \prime \right ) d\vz \prime + {\left (1 - \frac {1}{w^*}\right )}^{n} \, f\left (\vz \right ) &&\quad {\text {\textit {\cref {thm:lambda_bound}}}} \\ &\quad = n \, {\left (1 - \frac {1}{w^*}\right )}^{n-1} \Esub {q}{f} + {\left (1 - \frac {1}{w^*}\right )}^n \, f\left (\vz \right ). \end {alignat*}\end{proof}
\prAtEndRestatexii*
\label{proofsection:prAtEndxii}\begin{proof}[Proof of \autoref{thm:prAtEndxii}]\phantomsection\label{proof:prAtEndxii}\begin {alignat}{2} &\DTV {K^{k}\left (\veta , \cdot \right )}{\Pi } \nonumber \\ &\quad = \sup _{A} \abs { \Pi \left (A\right ) - P^{k}\left (\veta , A\right ) } &&\quad \text {\textit {Definition of \(d_{\text {TV}}\)}} \nonumber \\ &\quad \leq \sup _{A} \Bigg | \int _{A} \pi \left (d\vz \prime _1\right ) \times \ldots \times \pi \left (d\vz \prime _N\right ) \nonumber \\ &\qquad \qquad \qquad - K^{(k-1)\,N\,+1}\left (\vz _1, d\vz \prime _1\right ) \times \ldots \times K^{k\,N}\left (\vz _N, d\vz \prime _N\right ) \,\Bigg | \nonumber \\ &\quad \leq \sup _{A} \sum _{n=1}^N \abs { \int _{A} \pi \left (d\vz \prime _k\right ) - K^{(k-1)\,N + n}\left (\vz _n, d\vz \prime _n\right ) } &&\quad \text {\textit {\cref {thm:product_measure_bound}}} \nonumber \\ &\quad = \sum _{n=1}^N \DTV {K^{(k-1)\,N + n}\left (\vz _n, \cdot \right )}{\pi } &&\quad \text {\textit {Definition of \(d_{\text {TV}}\)}} \nonumber \\ &\quad \leq \sum _{n=1}^N \rho ^{(k-1)\,N + n} &&\quad \text {\textit {Geometric ergodicity}} \nonumber \\ &\quad = \rho ^{k\,N} \, \rho ^{-N} \, \frac {\rho - \rho ^{N+1}}{1 - \rho } &&\quad \text {\textit {Solved sum}} \nonumber \\ &\quad = \frac {\rho \, \left (1 - \rho ^N\right )}{\rho ^N \left (1 - \rho \right )} \, {\left ( \rho ^{N} \right )}^k \nonumber \end {alignat} \par \begin {alignat}{2} &\E { \norm { g\left (\cdot , \rvveta \right ) }^2_{*} \,\middle |\, \mathcal {F}_{t} } \nonumber \\ &\quad = \E { \norm { g\left (\cdot , \rvveta \right ) }^2 \,\middle |\, \vz _{t-1},\, \vlambda _{t-1} } \nonumber \\ &\quad = \E { \norm { \frac {1}{N}\sum ^{N}_{n=1} s\left (\cdot ; \rvvz _{n}\right ) }^2_{*} \,\middle |\, \vz _{t-1},\, \vlambda _{t-1} } \nonumber \\ &\quad \leq \E { \frac {1}{N^2} \sum ^{N}_{n=1} \norm {s\left (\cdot ; \rvvz _{n}\right ) }^2_{*} \,\middle |\, \vz _{t-1},\, \vlambda _{t-1} } &&\quad \text {\textit {Triangle inequality}} \nonumber \\ &\quad = \frac {1}{N^2}\sum ^{N}_{n=1} \Esub {\rvvz _{n} \sim K^n\left (\vz _{t-1}, \cdot \right )}{ \norm {s\left (\cdot ; \rvvz _{n}\right ) }^2_{*} \,\middle |\, \vz _{t-1},\, \vlambda _{t-1} } &&\quad \text {\textit {Linearity of expectation}} \nonumber \\ &\quad \leq \frac {1}{N^2}\sum ^{N}_{n=1} n \, {\left (1 - \frac {1}{w^*}\right )}^{n-1} \Esub {\rvvz _n \sim q_{\text {def.}}\left (\cdot ; \vlambda \right )}{ \norm {s\left (\cdot ; \rvvz _n \right )}_{*}^2 } \nonumber \\ &\qquad + {\left (1 - \frac {1}{w^*}\right )}^{n} \, \norm {s\left (\cdot ; \vz _{t-1} \right )}_{*}^2 &&\quad \text {\textit {\cref {thm:imh_expecation}}} \nonumber \\ &\quad \leq \frac {1}{N^2}\sum ^{N}_{n=1} n \, {\left (1 - \frac {1}{w^*}\right )}^{n-1} \, L^2 + {\left (1 - \frac {1}{w^*}\right )}^{n} \, L^2 \nonumber \\ &\quad = \frac {L^2}{N^2}\sum ^{N}_{n=1} n \, {\left (1 - \frac {1}{w^*}\right )}^{n-1} + {\left (1 - \frac {1}{w^*}\right )}^{n} \nonumber &&\quad \text {\textit {Moved constant forward}} \\ &\quad = \frac {L^2}{N^2} \, \left [\, {\left (w^*\right )}^2 + w^* - {\left (1 - \frac {1}{w^*}\right )}^N \left ( {\left (w^*\right )}^2 + w^* + N\,w^* \right ) \,\right ] \nonumber &&\quad \text {\textit {Solved sum}} \\ &\quad = \frac {L^2}{N^2} \, \left [\, \frac {1}{2} N^2 + \frac {3}{2}\,N + \mathcal {O}\left (1/w^*\right ) \,\right ] \nonumber &&\quad \text {\textit {Laurent series expansion at \(w \rightarrow \infty \)}} \\ &\quad = L^2 \, \left [\, \frac {1}{2} + \frac {3}{2}\,\frac {1}{N} + \mathcal {O}\left (1/w^*\right ) \,\right ] \nonumber \end {alignat} The laurent approximation is useful for realistic values of \(w^*\) since it is bounded below exponentially by the KL divergence.\end{proof}
\prAtEndRestatexiii*
\label{proofsection:prAtEndxiii}\begin{proof}[Proof of \autoref{thm:prAtEndxiii}]\phantomsection\label{proof:prAtEndxiii}For our new scheme, \begin {alignat}{2} &\DTV {K^{k}\left (\veta , \cdot \right )}{\Pi } \nonumber \\ &\quad = \sup _{A} \abs { \Pi \left (A\right ) - P^{k}\left (\veta , A\right ) } &&\quad \text {\textit {Definition of \(d_{\text {TV}}\)}} \nonumber \\ &\quad \leq \sup _{A} \big |\; \int _{A} \pi \left (d\vz \prime _1\right ) \cdot \ldots \cdot \pi \left (d\vz \prime _N\right ) \nonumber \\ &\qquad \qquad \qquad - K^k\left (\vz _1, d\vz \prime _1\right ) \cdot \ldots \cdot K^k\left (\vz _N, d\vz \prime _N\right ) \;\big | \nonumber \\ &\quad \leq \sup _{A} \sum _{n=1}^N \abs { \int _{A} \pi \left (d\vz \prime _k\right ) - K^{k}\left (\vz _n, d\vz \prime _n\right ) } &&\quad \text {\textit {\cref {thm:product_measure_bound}}} \nonumber \\ &\quad = \sum _{n=1}^N \DTV {K^k\left (\vz _n, \cdot \right )}{\pi } &&\quad \text {\textit {Definition of TV distance}} \nonumber \\ &\quad \leq \sum _{n=1}^N \rho ^{k} &&\quad \text {\textit {Geometric ergodicity}} \nonumber \\ &\quad = N\,\rho ^{k} &&\quad \text {\textit {Solved sum}} \nonumber \end {alignat} \par \begin {alignat}{2} &\E { \norm { g\left (\cdot , \rvveta \right ) }^2_{*} \,\middle |\, \mathcal {F}_{t} } \nonumber \\ &\quad = \E { \norm { g\left (\cdot , \rvveta \right ) }^2 \,\middle |\, \vz _{t-1}^{(1:N)},\, \vlambda _{t-1} } \nonumber \\ &\quad = \E { \norm { \frac {1}{N}\sum ^{N}_{n=1} s\left (\cdot ; \rvvz _{n}\right ) }^2_{*} \,\middle |\, \vz _{t-1}^{(1:N)},\, \vlambda _{t-1} } \nonumber \\ &\quad \leq \E { \frac {1}{N^2} \sum ^{N}_{n=1} \norm {s\left (\cdot ; \rvvz _{n}\right ) }^2_{*} \,\middle |\, \vz _{t-1}^{(1:N)},\, \vlambda _{t-1} } &&\quad \text {\textit {Triangle inequality}} \nonumber \\ &\quad = \frac {1}{N^2}\sum ^{N}_{n=1} \Esub {\rvvz _{n} \sim K\left (\vz _{t-1}^{(n)}, \cdot \right )}{ \norm {s\left (\cdot ; \rvvz _{n}\right ) }^2_{*} \,\middle |\, \vz _{t-1}^{(1:N)},\, \vlambda _{t-1} } &&\quad \text {\textit {Linearity of expectation}} \nonumber \\ &\quad \leq \frac {1}{N^2}\sum ^{N}_{n=1} \Esub {\rvvz _n \sim q_{\text {def.}}\left (\cdot ;\vlambda \right )}{ \norm {s\left (\cdot ; \rvvz _n \right )}_{*}^2 } + {\left (1 - \frac {1}{w^*}\right )} \, \norm {s\left (\cdot ; \vz _{t-1}^{(n)} \right )}_{*}^2 &&\quad \text {\textit {\cref {thm:imh_expecation}}} \nonumber \\ &\quad \leq \frac {1}{N^2}\sum ^{N}_{n=1} L^2 + {\left (1 - \frac {1}{w^*}\right )} \, L^2 \nonumber \\ &\quad = \frac {L^2}{N^2} \sum ^{N}_{n=1} 1 + {\left (1 - \frac {1}{w^*}\right )} \nonumber &&\quad \text {\textit {Moved constant forward}} \\ &\quad = L^2 \left [ \frac {1}{N} + \frac {1}{N}\,{\left (1 - \frac {1}{w^*}\right )} \right ]. \nonumber &&\quad \text {\textit {Solved sum}} \end {alignat}\end{proof}


==> preliminaries.tex <==

\begin{theoremEnd}{theorem}\label{thm:imh_exact_kernel}(\citealt[Theorem 1]{Smith96exacttransition})
  The \(t\)-step marginal IMH transition kernel is given as
  %\begin{align*}
  {\small
    \[
    K^t\left(\vz, d\vz^*\right) 
    = T_t\left(\, w\left(\vz\right) \vee w\left(\vz^*\right)\,\right) \, \pi\left(\vz^*\right) \, d\vz^*
    + \lambda^t\left(w\left(\vz\right)\right) \, \delta_{\vz}\left(d\vz^*\right)
    \]
  %\end{align*}
  }%
  where {\(w\left(\vz\right) = \pi\left(\vz\right)/q\left(\vz\right)\), \(x \vee y = \max\left(x, y\right)\)},
  {\small%
  \begin{align*}
  T_t\left(w\right)      = \int_w^{\infty} \frac{t}{v^2} \, \lambda^{t-1}\left(v\right)\,dv,\;\;
  \lambda\left(w\right) = \int_{R\left(w\right)} \left( 1 - \frac{w\left(\vz^*\right)}{w}  \right) \pi\left(d\vz^*\right)
  \end{align*}
  }
  for {\(R\left(w\right) = \{\, \vz^* \mid w\,\left(\vz^*\right) \leq w \,\}\)}.
\end{theoremEnd}

%%% Local Variables:
%%% TeX-master: "master"
%%% End:


==> prop_assumption.tex <==

\begin{theoremEnd}{proposition}\label{thm:imh_tail}
  For \(w\left(\vz\right) = \pi\left(\vz\right)/q\left(\vz\right)\) and the initial state \(\vz_0\), let \(w\left(\vz_0\right) > \epsilon\) and \(\pi\left(\vz_0\right) > \epsilon\) for some constant \(\epsilon > 0\).
  Then, the ratio between the \(t\)-step marginal kernel and the invariant distribution is bounded as
  {%\small
  \[
  \frac{K^t\left(\vz_0, \vz^*\right)}{\pi\left(\vz^*\right)} \leq
  \frac{t}{\epsilon} \, {\left(1 - \frac{1}{w^*}\right)}^{t-1}.
    %% \max\left\{\;
    %% \frac{t}{w^*} \, {\left(1 - \frac{1}{w^*}\right)}^{t-1},
    %% \frac{1}{\pi\left(\vz\right)} \, {\left(1-\frac{1}{w^*}\right)}^t
    %% \;\right\},
  \]
  }
  which is finite for all \(t\) if \(w^* < \infty\) where \(w^* = \sup_{\vz} w\left(\vz\right)\).
\end{theoremEnd}
\begin{proofEnd}
  Since the kernel \(K\) is a mixture of the accept and reject cases, 
  \begin{align}
    \frac{K^t\left(\vz_0, \vz^*\right)}{\pi\left(\vz^*\right)}
    &\leq
    \max\Bigg\{
    \underbrace{
      \frac{T_t\left(w\left(\vz_0\right) \vee w\left(\vz^*\right)\right)}{\pi\left(\vz^*\right)}
    }_{\text{accept}},
    \underbrace{
    \frac{\lambda^t\left(w\left(\vz_0\right)\right)}{\pi\left(\vz_0\right)}
    }_{\text{reject}}
    \Bigg\}
    &\text{(\cref{thm:imh_exact_kernel})}.\label{eq:prop_assumption_ratio}
  \end{align}
  For the accept case,
  \begin{align}
    \frac{T_t\left(w\left(\vz_0\right) \vee w\left(\vz^*\right)\right)}{\pi\left(\vz^*\right)}
    &\leq
    \frac{t}{w\left(\vz_0\right) \vee w\left(\vz^*\right)} \, {\left(1 - \frac{1}{w^*}\right)}^{t-1}
    &\text{(\cref{thm:tn_bound})}
    \\
    &\leq
    \frac{t}{\epsilon} \, {\left(1 - \frac{1}{w^*}\right)}^{t-1} .
  \end{align}
  and for the reject case,
  \begin{align}
    \frac{\lambda^t\left(w\left(\vz_0\right)\right)}{\pi\left(\vz\right)}
    \leq
    \frac{\lambda^t\left(w\left(\vz_0\right)\right)}{\pi\left(\vz\right)}
    \leq
    \frac{1}{\pi\left(\vz_0\right)} {\left(1 - \frac{1}{w^*}\right)}^{t}
    \leq
    \frac{1}{\epsilon}
    {\left(1 - \frac{1}{w^*}\right)}^{t}.
  \end{align}
  Therefore,~\cref{eq:prop_assumption_ratio} becomes
  \begin{align}
    \frac{K^t\left(\vz_0, \vz^*\right)}{\pi\left(\vz^*\right)}
    \leq
    \max\left\{\;
    \frac{t}{\epsilon} \, {\left(1 - \frac{1}{w^*}\right)}^{t-1},
    \frac{1}{\epsilon} \, {\left(1-\frac{1}{w^*}\right)}^t
    \;\right\}
    &\leq
    \frac{t}{\epsilon} \, {\left(1 - \frac{1}{w^*}\right)}^{t-1},
  \end{align}
  where the last inequality follows from \(1 - \frac{1}{w^*} \leq 1\)
\end{proofEnd}

%%% Local Variables:
%%% TeX-master: "master"
%%% End:


==> simulations.tex <==

\subsection{Isotropic Gaussian Experiments}
\begin{figure}[H]
  \centering
  \subfloat[\(N=2^2\)]{
    \includegraphics[scale=0.75]{figures/gaussian_01.pdf}
  }
  \subfloat[\(N=2^4\)]{
    \includegraphics[scale=0.75]{figures/gaussian_02.pdf}
  }
  \subfloat[\(N=2^6\)]{
    \includegraphics[scale=0.75]{figures/gaussian_03.pdf}
  }
  \caption{100-D isotropic Gaussian example with a varying computational budget \(N\).
    MSC-PIMH converges faster than MSC-CIS and MSC-CISRB regardless of \(N\).
    Also, the convergence of MSC-PIMH becomes more stable/monotonic as \(N\) increases.
    The solid lines and colored regions are the medians and 80\% percentiles computed from 100 repetitions.
  }\label{fig:gaussian}
\end{figure}
%
We perform experiments with a 100-D isotropic multivariate Gaussian distribution.
With Gaussian distributions, convergence can be evaluated exactly since their KL divergence is available in a closed form.
We compare the performance of MSC-PIMH, MSC-CIS, and MSC-CISRB with respect to the \(N\) (number of proposals for MSC-CIS, MSC-CISRB; number of parallel chains for MSC-PIMH).
The results are shown in~\cref{fig:gaussian}.
While MSC-PIMH shows some level of overshoot wih \(N=4\), it shows monotonic convergence with larger \(N\).
On the other hand, both MSC-CIS and MSC-CISRB overshoots even with \(N=64\).
This clearly shows that PIMH enjoys better gradient estimates compared to the CIS kernel.

\section{Numerical Simulation}
We present numerical simulations of our analyses in~\cref{section:bias_variance} and~\cref{section:cis_bias}.
In particular, we visualize the fact that the variance of the CIS kernel can increase with the number of proposals \(N\) when the KL divergence is large, as described in~\eqref{eq:cis_variance_incr}.

\paragraph{Experimental Setup}
We first set the target distribution as \(p\,(z \mid x) = \mathcal{N}(0, 1)\) and the proposal distribution as \(q\,(z; \mu) = \mathcal{N}(\mu, 2)\) with varying mean.
We measure the variance of estimating the score function \(s\,(z, \mu) = \frac{\partial q(\vz; \mu)}{\partial \mu} \) using the CIS, CISRB, and PIMH kernels, given the previous Markov-chain  denoted bystate \(z_{t-1}\) and computational budget \(N\).
For CIS and CISRB, we set a fixed \(z_{t-1}\), while for PIMH, we randomly sample \(N\) samples from \(\vz_{t-1} \sim p\,(z \mid z)\) (we obtained similar trends regardless of the distribution of \(z_{t-1}\)).
The variance is estimated using \(2^{14}\) samples from \(K(\vz_{t-1}, \cdot)\).
We report the variance across varying \(N\) and varying KL divergence between \(q_{\vlambda}(z)\) and \(p\,(\vz\mid\vx)\).
The latter is performed by varying the difference between the mean of the proposal and the target distributions denoted by \(\Delta \mu = \Esub{p(\vz\mid\vx)}{z} - \Esub{q_{\vlambda}}{z} \).

\begin{figure}[H]
  \centering
  \subfloat[\(\Delta \mu = 0\)]{
    \includegraphics[scale=0.75]{figures/simulations_01.pdf}
  }
  \subfloat[\(\Delta \mu = 2\)]{
    \includegraphics[scale=0.75]{figures/simulations_02.pdf}
  }
  \subfloat[\(\Delta \mu = 4\)]{
    \includegraphics[scale=0.75]{figures/simulations_03.pdf}
  }
  \caption{Conditional variance of different MCMC kernels with varying \(N\) and varying difference between the mean of the target and proposal distributions.
  }\label{fig:simulations}
  \vspace{-0.1in}
\end{figure}

\paragraph{Results Summary}
The results are presented in~\cref{fig:simulations}.
We can see that, when the difference of the mean of the \(p\) and \(q\) is large, the variance of CISRB \textit{increases} with \(N\).
This increasing trend becomes stronger as the KL divergence between \(p\) and \(q\) increases.
While this simulation suggests that CISRB has much smaller variance compared to CIS, our realistic experiments in~\cref{section:eval} did not reveal such levels of performance gains.
Is also visible that PIMH has a slightly larger variance compared to CIS in the small \(N\) regime.
This is due to the higher acceptance rate of the Metropolis-Hastings acceptance ratio used by PIMH compared to Barker's acceptance ratio used by CIS~\citep{peskun_optimum_1973, minh_understanding_2015}.

%%% Local Variables:
%%% TeX-master: "master"
%%% End:


==> thm_convergence_rate.tex <==

\begin{theoremEnd}[all end]{lemma}\label{thm:mixing_time}
  Assuming the kernel \(P_{\vlambda}\left(\veta, \cdot\right)\) satisfies \cref{thm:ergodicity}, the Hellinger mixing time \(\tau_{\text{Hel.}}\) is bounded as
  \begin{align*}
    \tau_{\text{Hel.}}\left(K_{\vlambda}, \epsilon\right) \leq  \frac{2}{\log \rho^{-1}} \log \frac{1}{\epsilon}
  \end{align*}
\end{theoremEnd}
\begin{proofEnd}
  The following two inequalities are equivalent.
  \begin{align*}
    d_{\text{Hel.}}\left(\, P^t_{\vlambda}\left(\veta, \cdot \right), \Pi \,\right)
    &\leq \sqrt{\DTV{ P^t_{\vlambda}\left(\veta, \cdot \right)}{\Pi}}
    \leq \rho^{t / 2}
    \\
    \log d_{\text{Hel.}}\left(\, P^t_{\vlambda}\left(\veta, \cdot \right), \Pi \,\right)
    &\leq \frac{t}{2} \log \rho
  \end{align*}

  The Hellinger mixing time \(\tau_{\text{Hel.}}\left(K_{\vlambda}, \epsilon\right)\) is the smallest \(t\) that statisfies the inequality
  \begin{align*}
    d_{\text{Hel.}}\left(\, P^t_{\vlambda}\left(\veta, \cdot \right), \Pi \,\right)
    &\leq 
    \epsilon.
  \end{align*}
  Instead, we can find the \(t\prime > t\) that satisfies
  \begin{align*}
    \log d_{\text{Hel.}}\left(\, P^t_{\vlambda}\left(\veta, \cdot \right), \Pi \,\right)
    \leq 
    \frac{t\prime}{2} \log \rho
    \leq 
    \log \epsilon
 \end{align*}
  by solving the inequalities
  \begin{alignat*}{2}
    \frac{t\prime}{2} \log \rho
    &\leq 
    \log \epsilon
    \\
    t\prime 
    &\geq 
    \frac{2}{\log \rho} \log \epsilon
    &&\quad\text{\textit{Inequality flipped since \(\log \rho \leq 1\)}}
    \\
    t\prime 
    &\geq 
    \frac{2}{\log \rho^{-1}} \log \frac{1}{\epsilon}
 \end{alignat*}
\end{proofEnd}

\begin{theoremEnd}{theorem}{(\textbf{Convergence rate})}\label{thm:convergence_rate}
  Assuming~\cref{thm:kernel_conditions,thm:gradient_estimator,thm:logconcave,thm:compact,thm:bounded_variance} hold, with a diminishing stepsize of \(\alpha_t = \alpha /  \sqrt{T} \), the average iterates {\small\(\overline{\vlambda}_T = \sum^{T}_{t=1} \vlambda_{t} / T\)} of Markov chain score ascent achieve a convergence rate of
  {%\small
  \begin{align*}
    \E{ \DKL{\pi}{q\,(\cdot; {\overline{\vlambda}_{T}})} - \DKL{\pi}{q\left(\cdot; {\vlambda^*}_{T}\right)}}
    =
    \mathcal{O}\left(
    \frac{
      \alpha \, G^2 \, \sqrt{\log T}
    }{
      \log \rho^{-1} \, \sqrt{T}
    } \right)  
  \end{align*}
  }
\end{theoremEnd}
\begin{proofEnd}
  \citet[Corollary 3.5]{duchi_ergodic_2012} provide a non-asymptotic convergence rate for the \textit{ergodic mirror descent} algorithm which computes the parameter update as
  \begin{align}
    \vlambda_{t+1} &= \argmin_{\vlambda \in \Lambda} \left\{\,
    \iprod{\,\vg\left(\vlambda, \veta_t\right)}{\vlambda\,} 
    +
    \frac{1}{\alpha_t} D_{\psi}\left(\vlambda, \vlambda_{t}\right)
    \,\right\}\label{eq:ergodic_mirror_descent}
    \\
    \rvveta_{t+1} &\sim P_{\vlambda_{t}}\left(\veta_t, \cdot\right)
    \nonumber
  \end{align}
  where \(D_{\psi}\) is the Bregman divergence defined as
  \begin{align*}
    D_{\psi}\left(\vlambda, \vlambda\prime\right)
    \triangleq
    \psi\left(\vlambda\right)
    - \psi\left(\vlambda\prime\right)
    - \iprod{ \nabla \psi\left(\vlambda\prime\right)}{\vlambda - \vlambda\prime}
  \end{align*}
  for some convex function \(\psi\).
  Our result is based on the fact that MCGD is a special case of the ergodic mirror descent algorithm.
  Specifically, by choosing \(\psi\left(\vlambda\right) = \frac{1}{2} \norm{\vlambda}^2_2 \), we obtain
  \begin{alignat}{2}
    D_{\psi}\left(\vlambda, \vlambda\prime\right) = \frac{1}{2} \norm{\vlambda - \vlambda\prime}_2^2 \leq \frac{1}{2} \, R^2.\label{eq:bregman}
    &&\quad\text{\textit{\cref{thm:compact}}}
  \end{alignat}
  This reduces the update in \cref{eq:ergodic_mirror_descent} into projected gradient descent which is the form used for Markov chain score climbing.

  Under our assumptions, \citet[Corollary 3.5]{duchi_ergodic_2012} show that, by assuming that the Hellinger mixing time is bounded as
  \begin{align}
    \tau_{\text{Hel.}}\left(K_{\vlambda}, \epsilon\right) \leq \kappa_1 \log\left( \kappa_2 /\epsilon \right) \label{eq:hellinger_mixing}
  \end{align}
  for any \(\epsilon > 0\), and setting a decreasing stepsize \(\alpha_t = \alpha / \sqrt{t}\),
  it follows that
  \begin{align}
    &\E{ \DKL{\pi}{q\,(\cdot; {\overline{\vlambda}_{T}})} - \DKL{\pi}{q\left(\cdot; {\vlambda^*}_{T}\right)}}
    \nonumber
    \\
    &\;\leq
    \frac{R^2}{2 \, \alpha \, \sqrt{T}}
    +
    \frac{2 \, \alpha \, G^2}{\sqrt{T}}\left( \kappa_1 \, \log \frac{\kappa_2}{\epsilon} \right)
    +
    3 \, \epsilon \, G \, R
    +
    \frac{R \, G \, \kappa_1 \, \log \frac{\kappa_2}{\epsilon}}{T}.
    \label{eq:duchi_base}
  \end{align}

  From \cref{thm:mixing_time}, we retrieve the constants of \cref{eq:hellinger_mixing} as
  \(
  \kappa_1=\frac{2}{\log \rho^{-1} },\;  \kappa_2 = 1
  \), and set \(\epsilon = 1/\sqrt{T}\).
  Then, using
  \begin{alignat}{2}
    \kappa_1 \, \log \frac{\kappa_2}{\epsilon}
    =
    \frac{1}{\log \rho^{-1} } \, \log T,\label{eq:kappa}
  \end{alignat}
  it follows that
  \begin{alignat*}{2}
    &\E{ \DKL{\pi}{q\,(\cdot; {\overline{\vlambda}_{T}})} - \DKL{\pi}{q\left(\cdot; {\vlambda^*}_{T}\right)}}
    \\
    &\;\leq
    \frac{R^2}{2 \, \alpha \, \sqrt{T}}
    +
    \frac{2 \, \alpha \, G^2}{\sqrt{T}}\left( \kappa_1 \, \log \frac{\kappa_2}{\epsilon} \right)
    +
    3 \, \epsilon \, G \, R
    +
    \frac{R \, G \, \kappa_1 \, \log \frac{\kappa_2}{\epsilon}}{T}.
    \nonumber
    &&\quad\text{\textit{\cref{eq:duchi_base}}}
    \\
    &\;=
    \frac{R^2}{2 \, \alpha \, \sqrt{T}}
    +
    \frac{2 \, \alpha \, G^2 \, \log T }{\log \rho^{-1} \, \sqrt{T}}
    +
    3 \, \epsilon \, G \, R
    +
    \frac{R \, G \, \log T }{\log \rho^{-1} \, T}.
    \nonumber
    &&\quad\text{\textit{\cref{eq:kappa}}}
  \end{alignat*}
\end{proofEnd}

%%% Local Variables:
%%% TeX-master: "master"
%%% End:


==> thm_convergence_rate2.tex <==

\begin{theoremEnd}{theorem}{(\textbf{Convergence rate})}\label{thm:convergence_rate}
\end{theoremEnd}
\begin{proofEnd}
  \begin{alignat}{2}
    \norm{
      \vlambda_{t+1} - \vlambda^*
    }^2
    &=
    \norm{
      \vlambda_{t} - \alpha_t \, \vg\left(\lambda_t, \eta_t\right)  - \vlambda^*
    }^2
    \\
    &=
    \norm{
      \vlambda_{t} - \vlambda^*
    }^2
    -2 \alpha_k \iprod{
      \, \vg\left(\vlambda_t, \eta_t\right)
    }{
      \vlambda_{t} - \vlambda^* \,
    }
    +
    \alpha_k^2 \norm{
      \vg\left(\vlambda_t, \eta_t\right)
    }
  \end{alignat}

  \begin{alignat}{2}
    f\left(\vy\right) - f\left(\vx\right) \leq - \iprod{\nabla f\left(\vx\right)}{\vx - \vy}
  \end{alignat}

  \begin{alignat}{2}
    f\left(\vy\right) \geq f\left(\vx\right) + \iprod{\nabla f\left(\vx\right)}{\vy - \vx} + \frac{\mu}{2} \norm{\vy - \vx}^2
  \end{alignat}

  \begin{alignat}{2}
    &-2 \alpha_t \iprod{
      \, \vg\left(\vlambda_t, \eta_t\right)
    }{
      \vlambda_{t} - \vlambda^* \,
    }
    \\
    &\;=
    -2 \alpha_t \iprod{
      \, \vg\left(\vlambda_t, \eta_t\right)
      - \nabla f\left(\vlambda_t\right)
    }{
      \vlambda_{t} - \vlambda^* \,
    }
    -2 \alpha_t \iprod{
      \nabla f\left(\vlambda_t\right)
    }{
      \vlambda_{t} - \vlambda^* \,
    }
    \\
    &\;\leq
    -2 \alpha_t \iprod{
      \, \vg\left(\vlambda_t, \eta_t\right)
      - \nabla f\left(\vlambda_t\right)
    }{
      \vlambda_{t} - \vlambda^* \,
    }
    -2 \alpha_t \left( f\left(\vlambda_t\right) - f\left(\vlambda^*\right) \right)
    \\
    &\;\leq
    2 \alpha_t
    \norm{
      \vg\left(\vlambda_t, \eta_t\right) - \nabla f\left(\vlambda_t\right)
    }_{*} \,
    \norm{
      \vlambda_{t} - \vlambda^* 
    }
    -2 \alpha_t \left( f\left(\vlambda_t\right) - f\left(\vlambda^*\right) \right)
  \end{alignat}
\end{proofEnd}

%%% Local Variables:
%%% TeX-master: "master"
%%% End:


==> thm_gradient_bound.tex <==

\begin{theoremEnd}{proposition}\label{thm:score_bound}
  The score gradient of the variational approximation \(q\left(\cdot; \vlambda\right)\) in the location scale family with a base density that is uniformly Lipschitz continuous as
  \begin{align*}
    \norm{ \nabla_{\vlambda} \log q\left(\cdot; \vlambda\right) }_2
    \leq
    D \, L \, M \left( \norm{\vz}_2 + \norm{\vlambda}_2 + 1 \right)
  \end{align*}
  where \(\vz \in \mathbb{R}^D\).
\end{theoremEnd}
\begin{proofEnd}
  Let us denote the reparameterization function 
  \begin{align}
    \vt^{-1}\left(\vz, \vlambda\right) = \mC^{-1}_{\vlambda}\left(\vz - \vm_{\vlambda}\right)\label{eq:reparam}
  \end{align}
  such that
  \begin{align*}
    q\left(\vz; \vlambda\right) = \phi\left( \vt^{-1}\left(\vz, \vlambda\right) \right).
  \end{align*}

  for \(\vlambda = (\vm_{\vlambda}, \mC_{\vlambda})\), \(\vmu = (\vm_{\vmu}, \mC_{\vmu})\)
  Using this, we analyze the gradient of the location \(\vm_{\vlambda}\) and scale \(\mC_{\vlambda}\) parameters separately.
  First, the gradient of the location parameter is bounded as
  \begin{alignat}{2}
    \norm{
      \nabla_{\vm_{\vlambda}} \log q\left(\vz; \vlambda\right)
    }_2
    &=
    \norm{
      \nabla_{\vm_{\vlambda}} \log \phi\left( \vt^{-1}\left(\vz, \vlambda\right) \right)
    }_2
    &&\quad\text{\textit{\cref{eq:reparam}}}
    \nonumber
    \\
    &=
    \norm{
    \nabla_{\vm_{\vlambda}} \vt^{-1}\left(\vz, \vlambda\right)  \nabla_{\vt^{-1}} \log \phi\left( \vt^{-1}\left(\vz, \vlambda\right) \right) 
    }_2
    &&\quad\text{\textit{Chain rule}}
    \nonumber
    \\
    &=
    \norm{
    \nabla_{\vm_{\vlambda}} \left( \mC^{-1}_{\vlambda}\left(\vz - \vm_{\vlambda}\right) \right) \nabla_{\vt^{-1}} \log \phi\left( \vt^{-1}\left(\vz, \vlambda\right) \right) 
    }_2
    &&\quad\text{\textit{\cref{eq:reparam}}}
    \nonumber
    \\
    &=
    \norm{
      -\mC^{-1}_{\vlambda}
      \nabla_{\vt^{-1}} \log \phi\left( \vt^{-1}\left(\vz, \vlambda\right) \right) 
    }_2
    &&\quad\text{\textit{Solved derivative}}
    \nonumber
    \\
    &\leq
    \norm{
      \mC^{-1}_{\vlambda}
    }_{\mathrm{op}}
    \,
    \norm{
      \nabla_{\vt^{-1}} \log \phi\left( \vt^{-1}\left(\vz, \vlambda\right) \right) 
    }_2
    \nonumber
    \\
    &\leq
    \sqrt{M} \,
    L.
    &&\quad\text{\textit{\cref{thm:lipschitz}}}
    \label{eq:location_grad}
  \end{alignat}

  Second, for the scale parameter, we bound the derivative of the \(i,j\) element of the matrix \(\mC_{\vlambda}\).
  Let us drop the subscript \(\vlambda\) for clarity.
  Then, similarly to the location parameter,
  \begin{alignat}{2}
    \abs{
      \nabla_{\mC_{i,j}} \log q\left(\vz; \vlambda\right)
    }
    &=
    \abs{
      \nabla_{\mC_{i,j}} \log \phi\left( \vt^{-1}\left(\vz, \vlambda\right) \right)
    }
    &&\quad\text{\textit{\cref{eq:reparam}}}
    \nonumber
    \\
    &=
    \abs{
      \iprod{
        \nabla_{\mC_{i,j}} \vt^{-1}\left(\vz, \vlambda\right)   
      }{
        \nabla_{\vt} \log \phi\left( \vt^{-1}\left(\vz, \vlambda\right) \right)   
      }
    }
    &&\quad\text{\textit{Chain rule}}
    \nonumber
    \\
    &=
    \abs{
      \iprod{
        \nabla_{\mC_{i,j}} \left( \mC^{-1}_{\vlambda}\left(\vz - \vm_{\vlambda}\right) \right)
      } {
        \nabla_{\vt} \log \phi\left( \vt^{-1}\left(\vz, \vlambda\right) \right)          
      }
    }
    \nonumber
    \\
    &\leq
    \norm{
      \nabla_{\mC_{i,j}} \left( \mC^{-1}_{\vlambda}\left(\vz - \vm_{\vlambda}\right) \right)
    }_2 \,
    \norm{
      \nabla_{\vt} \log \phi\left( \vt^{-1}\left(\vz, \vlambda\right) \right)          
    }_2
    &&\quad\text{\textit{Cauchy-Schwarz inequality}}
    \nonumber
    \\
    &\leq
    L\,
    \norm{
      \nabla_{\mC_{i,j}} \left( \mC^{-1}_{\vlambda}\left(\vz - \vm_{\vlambda}\right) \right)
    }_2.
    &&\quad\text{\textit{\cref{thm:lipschitz}}}
    \nonumber
    \\
    &=
    L\,
    \norm{
    \mC^{-1}_{\vlambda} \frac{\partial \mC}{\partial_{\mC_{i,j}}} \mC^{-1}_{\vlambda}  \left(\vz - \vm_{\vlambda}\right) 
    }_2
    \nonumber
    &&\quad\text{\textit{Solved gradient}}
    \\
    &\leq
    L\,
    \norm{
      \mC^{-1}_{\vlambda}
    }_{\text{op}} \,
    \norm{
      \frac{\partial \mC}{\partial_{\mC_{i,j}}}
    }_{\text{op}} \,
    \norm{
      \mC^{-1}_{\vlambda} 
    }_{\text{op}}
    \norm{
    \vz - \vm_{\vlambda}
    }_2
    \nonumber
    &&\quad\text{\textit{Property of operator norm}}
    \\
    &=
    L\,
    \norm{
      \mC^{-1}_{\vlambda}
    }_{\text{op}} \,
    \norm{
      \mC^{-1}_{\vlambda} 
    }_{\text{op}}
    \norm{
    \vz - \vm_{\vlambda}
    }_2
    &&\quad\text{\textit{Largest eigenvalue \(\sigma_{\text{max}}\left(\frac{\partial \mC}{\partial_{\mC_{i,j}}}\right) = 1\)}}
    \nonumber
    \\
    &\leq
    L \,
    M \,
    \norm{
    \vz - \vm_{\vlambda}
    }_2
    &&\quad\text{\textit{\cref{thm:solution_space}}}
    \nonumber
    \\
    &\leq
    L \,
    M \,\left(
    \norm{\vz}_2 + \norm{\vm_{\vlambda}}_2
    \right)
    &&\quad\text{\textit{Triangle inequality}}
    \nonumber
    \\
    &\leq
    L \,
    M \, \left(
    \norm{\vz}_2 + \norm{\vlambda}_2
    \right)
    &&\quad\text{\textit{\cref{eq:parameter_norm}}}
    \nonumber
  \end{alignat}

  Now, by the poperty of norms,
  \begin{alignat}{2}
    \norm{
      \nabla_{\mC} \log q\left(\vz; \vlambda\right)
    }_{F}
    &\leq
    D \,
    \sup_{i,j}
    \abs{
      \nabla_{\mC_{i,j}} \log q\left(\vz; \vlambda\right)
    }
    \nonumber
    \\
    &\leq
    D \,
    L \,
    M \, \left(
    \norm{\vz} + \norm{\vlambda}
    \right).
    \label{eq:scale_grad}
  \end{alignat}
  Then, combining \cref{eq:location_grad,eq:scale_grad}, 
  \begin{alignat}{2}
    \norm{
      \nabla_{\vlambda} \log q\left(\vz; \vlambda\right)
    }
    &\leq
    \norm{
      \nabla_{\vm_{\vlambda}} \log q\left(\vz; \vlambda\right)
    }_2
    +
    \norm{
      \nabla_{\mC_{\vlambda}} \log q\left(\vz; \vlambda\right)
    }_{F} 
    &&\quad\text{\textit{\cref{eq:parameter_norm}}}
    \nonumber
    \\
    &\leq
    D \,
    L \,
    M \, \left(
    \norm{\vz}_2 + \norm{\vlambda}_2
    \right)
    +
    \sqrt{M} \, L
    &&\quad\text{\textit{\cref{eq:location_grad,eq:scale_grad}}}
    \nonumber
    \\
    &\leq
    D \,
    L \,
    M \, \left(
    \norm{\vz}_2 + \norm{\vlambda}_2
    +
    1 
    \right).
    \nonumber
  \end{alignat}
\end{proofEnd}

%%% Local Variables:
%%% TeX-master: "master"
%%% End:


==> thm_log_concave.tex <==


\begin{theoremEnd}[all end]{lemma}\label{thm:additive}
  The bivariate function location and scale reparameterization function
  \(
    t\left(\vu, \vlambda\right) = \mC\,\vu + \vm
  \)
  is additive with respect to \(\vlambda =\left[\mC, \vm\right]\) such that
  \[
    t\left(\vu, \alpha\,\vlambda + \beta\,\vmu\right) 
    = \alpha\,t\left(\vu, \vlambda\right) + \beta\,t\left(\vu, \vmu\right)
  \]
  for any \(\alpha\), \(\beta\).
\end{theoremEnd}
\begin{proofEnd}
  Let us denote \(\vlambda =\left[\mC_{\vlambda}, \vm_{\vlambda}\right]\) and \(\vmu = \left[\mC_{\vmu}, \vm_{\vmu}\right]\).
  Then,
  \begin{alignat}{2}
    t\left(\vu, \alpha\,\vlambda + \beta\,\vmu\right) 
    &= 
    \left(\alpha\,\mC_{\vlambda} + \beta\,\mC_{\vmu}\right)\,\vu + \left(\alpha\,\vm_{\vlambda} + \beta\,\vm_{\vmu}\right)
    \nonumber
    \\
    &= 
    \alpha\,\left(\mC_{\vlambda}\vu + \vm_{\vlambda}\right) + \beta\,\left(\mC_{\vmu}\,\vu + \vm_{\vmu}\right)
    \nonumber
    \\
    &= 
    \alpha\,t\left(\vu, \vlambda\right) + \beta\,t\left(\vu, \vmu\right).
    \nonumber
  \end{alignat}
\end{proofEnd}

\begin{theoremEnd}{proposition}\label{thm:logconcave_parameter}
  Any location-scale log-concave family is log-concave with respect to its location and scale parameters.
\end{theoremEnd}
\begin{proofEnd}
  A distribution \(q\left(\cdot\right) \in \mathcal{Q}\) in a location-scale family \(\mathcal{Q}\) is defined as
  \begin{align*}
    \rvvz \sim q\left(\cdot\right) \iff \rvvz = t\left(\rvvu, \vlambda\right),\; \rvvu \sim \phi\left(\cdot\right).
  \end{align*}
  The reparameterization function \(t\) is defined as an affine transformation
  \begin{align*}
    t\left(\vu, \vlambda\right) = \mC\,\vu + \vm
  \end{align*}
  for the location \(\vm\) and scale \(\mC\) parameters and their concatenation \(\vlambda = \left[\mC, \vm\right]\).

  Furthermore, the base density \(\phi\left(\vz\right)\) of any location-scale log-concave family is log-concave.
  Therefore, it follows that
  \begin{alignat}{2}
    &\log\phi\left(t\left(\vu, \alpha \vlambda + (1 - \alpha)\,\vmu\right)\right)
    \nonumber
    \\
    &\quad=
    \log\phi\left( \alpha\,t\left(\vu, \vlambda\right) + (1 - \alpha)\,t\left(\vu, \vmu\right)\right)
    &&\quad\text{\textit{\cref{thm:additive}}}
    \nonumber
    \\
    &\quad=
    \alpha\,\log\phi\left(t\left(\vu, \vlambda\right)\right) + (1 - \alpha)\,\log\phi\left(t\left(\vu, \vmu\right)\right)
    &&\quad\text{\textit{Log-concavity of \(\phi\)}}.
    \nonumber
  \end{alignat}
\end{proofEnd}

%%% Local Variables:
%%% TeX-master: "master"
%%% End:


==> thm_strongly_log_concave.tex <==

\begin{theoremEnd}[all end]{lemma}\label{thm:reparam_function}
  For the inverse location and scale reparameterization function
  \(
    t^{-1}\left(\vu, \vlambda\right) = \mC^{-1}_{\vlambda}\,\left( \vz - \vm_{\vlambda} \right)
  \),
  it follows that
  \begin{align*}
    \vt^{-1}\left(\vu, \alpha\,\vlambda + \left(1 - \alpha\right)\,\vmu\right) 
    = \;
    &\alpha \, \vt^{-1}\left(\vz, \vlambda\right) + \left(1 - \alpha\right) \, \vt^{-1}\left(\vz, \vmu\right)
    \\
    &\; + \alpha \left(1 - \alpha\right) \, \left(\mC^{-1}_{\vlambda}  - \mC^{-1}_{\vmu} \right)\, \left(\vm_{\vlambda} - \vm_{\vmu} \right)
  \end{align*}
  for any \(0 < \alpha < 1\).
\end{theoremEnd}
\begin{proofEnd}
  Let us denote \(\vlambda =\left(\mC_{\vlambda}, \vm_{\vlambda}\right)\) and \(\vmu = \left(\mC_{\vmu}, \vm_{\vmu}\right)\).
  Then, from the definition of \(\vt\),
  \begin{alignat}{2}
    \vt^{-1}\left(\vz, \alpha\,\vlambda + \beta\,\vmu\right) 
    &=
    \left(\alpha \, \mC^{-1}_{\vlambda} + (1 - \alpha)\,\mC^{-1}_{\vmu} \right) \, \big(\vz - ( \alpha\,\vm_{\vlambda} + (1 - \alpha)\, \vm_{\vmu} )  \big)
    \nonumber
    \\
    &= \textcolor{purple}{\left(\alpha \, \mC^{-1}_{\vlambda} + (1 - \alpha)\,\mC^{-1}_{\vmu} \right) \, \vz} \textcolor{orange}{
      - \left(\alpha \, \mC^{-1}_{\vlambda} + (1 - \alpha)\,\mC^{-1}_{\vmu} \right) \, \left( \alpha\,\vm_{\vlambda} + (1 - \alpha)\, \vm_{\vmu} \right).
    }
    \label{eq:reparam_linear_main}
  \end{alignat}

  For the first term, 
  \begin{alignat}{2}
    &\textcolor{purple}{\left(\alpha \, \mC^{-1}_{\vlambda} + (1 - \alpha)\,\mC^{-1}_{\vmu} \right) \, \vz}
    \nonumber
    \\
    \nonumber
    &\;= \alpha \, \mC^{-1}_{\vlambda}  \, \vz + (1-\alpha) \, \mC^{-1}_{\vmu} \vz
    &&\quad\text{\textit{Distributed \(\vz\)}}
    \\
    &\;= \alpha \, \mC^{-1}_{\vlambda} \, \left( \vz \textcolor{blue}{ - \vm_{\vlambda}} \right) + \textcolor{blue}{ \alpha \, \mC^{-1}_{\vlambda} \,  \vm_{\vlambda}} + (1 - \alpha) \, \mC^{-1}_{\vmu} \left(\vz  \textcolor{blue}{ - \vm_{\vmu}}\right) + \textcolor{blue}{(1 - \alpha) \, \mC^{-1}_{\vmu} \, \vm_{\vmu}}
    &&\quad\text{\textit{Added \textcolor{blue}{redundant terms}}}
    \nonumber
    \\
    &\;= \alpha \, \vt^{-1}\left(\vz, \vlambda\right) + \textcolor{blue}{ \alpha \, \mC^{-1}_{\vlambda} \vm_{\vlambda} } + (1-\alpha) \, \vt^{-1}\left(\vz, \vmu\right) + \textcolor{blue}{ (1-\alpha) \, \mC^{-1}_{\vmu} \vm_{\vmu} }
    &&\quad\text{\textit{Definition of \(\vt^{-1}\)}}
    \label{eq:reparam_linear}
  \end{alignat}

  The redundant terms \textcolor{blue}{\(\alpha \, \mC^{-1}_{\vlambda} \, \vm_{\vlambda}\)} and \textcolor{blue}{ \((1-\alpha)\, \mC^{-1}_{\vmu} \, \vm_{\vmu}\)} are absorbed by the \textcolor{orange}{second term} of~\cref{eq:reparam_linear_main}.
  That is, from~\cref{eq:reparam_linear_main,eq:reparam_linear},
  \begin{alignat}{2}
    &\textcolor{blue}{\alpha \, \mC^{-1}_{\vlambda} \vm_{\vlambda} + (1-\alpha) \, \mC^{-1}_{\vmu} \vm_{\vmu}} \textcolor{orange}{ - \left(\alpha \, \mC^{-1}_{\vlambda} + (1-\alpha)\,\mC^{-1}_{\vmu} \right) \, \left( \alpha\,\vm_{\vlambda} + (1-\alpha)\, \vm_{\vmu} \right)}
    \nonumber
    \\
    &= \alpha \, \mC^{-1}_{\vlambda} \vm_{\vlambda}  + (1-\alpha) \, \mC^{-1}_{\vmu} \vm_{\vmu} + \left(\alpha \, \mC^{-1}_{\vlambda} + (1-\alpha)\,\mC^{-1}_{\vmu} \right) \, \left( -\alpha\,\vm_{\vlambda} -(1-\alpha)\, \vm_{\vmu} \right)
    &&\quad\text{\textit{Flipped sign of the last term}}
    \nonumber
    \\
    &= 
    \alpha \, \mC^{-1}_{\vlambda} \, \left(\vm_{\vlambda} - \alpha\,\vm_{\vlambda} - (1-\alpha)\, \vm_{\vmu} \right)
    +
    (1-\alpha) \, \mC^{-1}_{\vmu} \, \left(\vm_{\vmu} - \alpha\,\vm_{\vlambda} - (1-\alpha)\, \vm_{\vmu}  \right)
    &&\quad\text{\textit{Grouped terms with \(\mC^{-1}_{\vlambda}\) and \(\mC^{-1}_{\vmu}\)}}
    \nonumber
    \\
    &= 
    \alpha \, \mC^{-1}_{\vlambda} \, \left(\left(1 - \alpha\right)\vm_{\vlambda} - (1-\alpha)\, \vm_{\vmu} \right)
    +
    (1-\alpha) \, \mC^{-1}_{\vmu} \, \left(\alpha\,\vm_{\vmu} - \alpha\,\vm_{\vlambda} \right)
    &&\quad\text{\textit{Grouped terms with \(\vm_{\vlambda}\) and \(\vm_{\vmu}\)}}
    \nonumber
    \\
    &= \alpha \, (1-\alpha) \, \mC^{-1}_{\vlambda} \, \left(\vm_{\vlambda} - \vm_{\vmu} \right)
    +
    \alpha \, (1-\alpha) \, \mC^{-1}_{\vmu} \, \left(\vm_{\vmu} - \vm_{\vlambda}  \right)
    &&\quad\text{\textit{Pulled constants forward}}
    \nonumber
    \\
    &= 
    \alpha \, (1-\alpha) \, \left(\mC^{-1}_{\vlambda}  - \mC^{-1}_{\vmu} \right)\, \left(\vm_{\vlambda} - \vm_{\vmu} \right)
    \nonumber
  \end{alignat}
  We obtain our conclusion by combining this with \cref{eq:reparam_linear}.
\end{proofEnd}

\begin{theoremEnd}{proposition}\label{thm:logconcave_parameter}
  A multivariate Gaussian \(q\left(\cdot; \vlambda\right)\) in the solution space \(\vlambda \in \mathcal{\Lambda}_M\) is strongly log-concave with respect to its location and scale parameters.
\end{theoremEnd}
\begin{proofEnd}
  A probability density function in the multivariate Gaussian variational family can be represented as 
  \begin{align}
    q\left(\vz; \vlambda\right) &= \phi\left( \vt^{-1}\left(\vz, \vlambda\right) \right)
    \label{eq:gaussian_reparam}
  \end{align}
  where \(\phi\left(\cdot\right)\) is the unit multivariate Gaussian density, \(\vlambda = \left(\vm_{\vlambda}, \mC_{\vlambda}\right)\) is the concatenation of the location (\(\vm_{\vlambda}\)) and scale (\(\mC_{\vlambda}\)) parameters, and
  \begin{align}
    \vt\left(\vu, \vlambda\right)     &= \mC_{\vlambda} \vu + \vm_{\vlambda} \nonumber \\
    \vt^{-1}\left(\vz, \vlambda\right) &= \mC^{-1}_{\vlambda} \left(\vz - \vm_{\vlambda} \right)\label{eq:reparam}
  \end{align}
  is the location-scale reparameterization function.
  Furthermore, the unit multivariate Gaussian \(\phi\left(\cdot\right)\) is strongly log-concave as
  \begin{align}
    \log \phi\left(\vu\right) = -\frac{1}{2}\norm{\vu}^{2}_{2} - \log Z \label{eq:gaussian_norm}
  \end{align}
  where \(Z > 1\) is a normalizing constant.

  The location-scale reparameterization function~\cref{eq:reparam} has the property

  From this, for \(0 < \alpha < 1\), the strong log-concavity of the Gaussian follows as 
  \begin{alignat}{2}
    &\log q\left(\vz; \alpha\,\vlambda + (1 - \alpha)\,\vmu\right) 
    \nonumber
    \\
    &= \log \phi\left( \vt^{-1}\left(\vz, \alpha\,\vlambda + (1 - \alpha)\,\vmu\right) \right) 
    &&\quad\text{\textit{\cref{eq:gaussian_reparam}}}
    \nonumber
    \\
    &= -\frac{1}{2}\norm{\vt^{-1}\left(\vz, \alpha\,\vlambda + (1-\alpha)\,\vmu\right)}_2^2 - \log Z
    &&\quad\text{\textit{\cref{eq:gaussian_norm}}}
    \nonumber
    \\
    &= -\frac{1}{2}\norm{
      \alpha \, \vt^{-1}\left(\vz, \vlambda\right) + (1-\alpha) \, \vt^{-1}\left(\vz, \vmu\right)
      +
      \alpha \, (1-\alpha) \, \left(\mC^{-1}_{\vlambda}  - \mC^{-1}_{\vmu} \right)\, \left(\vm_{\vlambda} - \vm_{\vmu} \right)
    }_2^2 - \log Z
    &&\quad\text{\textit{\cref{thm:reparam_function}}}
    \nonumber
    \\
    &\geq
    -\frac{\alpha}{2}\norm{
      \vt^{-1}\left(\vz, \vlambda\right)
    }^2_2
    -\frac{(1-\alpha)}{2}\norm{
      \vt^{-1}\left(\vz, \vmu\right)
    }^2_2
    -\frac{\alpha \, (1-\alpha)}{2}\norm{
     \left(\mC^{-1}_{\vlambda}  - \mC^{-1}_{\vmu} \right)\, \left(\vm_{\vlambda} - \vm_{\vmu} \right)
    }_2^2 - 2\,\log Z
    &&\quad\text{\textit{Triangle inequality}}
    \nonumber
    \\
    &=
    \alpha \log \phi\left( \vt^{-1}\left(\vz, \vlambda\right) \right)
    +
    (1-\alpha) \log \phi\left( \vt^{-1}\left(\vz, \vmu\right) \right)
    -\frac{\alpha \, (1-\alpha)}{2}\norm{
     \left(\mC^{-1}_{\vlambda}  - \mC^{-1}_{\vmu} \right)\, \left(\vm_{\vlambda} - \vm_{\vmu} \right)
    }_2^2
    &&\quad\text{\textit{\cref{eq:gaussian_norm}}}
    \nonumber
    \\
    &=
    \alpha \, \log q\left(\vz; \vlambda \right)
    +
    (1-\alpha) \, \log q\left(\vz; \vmu\right)
    -\frac{\alpha \, (1-\alpha)}{2}\norm{
     \left(\mC^{-1}_{\vlambda}  - \mC^{-1}_{\vmu} \right)\, \left(\vm_{\vlambda} - \vm_{\vmu} \right)
    }_2^2
    &&\quad\text{\textit{\cref{eq:gaussian_reparam}}}
    \nonumber
  \end{alignat}
  The remaining term results in the smoothness as
  \begin{alignat}{2}
    &-\frac{\alpha \, (1-\alpha)}{2}\norm{
     \left(\mC^{-1}_{\vlambda}  - \mC^{-1}_{\vmu} \right)\, \left(\vm_{\vlambda} - \vm_{\vmu} \right)
    }_2^2
    \\
    &\;\geq
    -\frac{\alpha \, (1-\alpha)}{2}
    \norm{
      \mC^{-1}_{\vlambda}  - \mC^{-1}_{\vmu}
    }^2_{\mathrm{op}}
    \norm{
      \vm_{\vlambda} - \vm_{\vmu}
    }_2^2
    \nonumber
    \\
    &\;\geq
    -\frac{\alpha  \, (1-\alpha) \, }{2} \,
    \left(
    \norm{
      \mC^{-1}_{\vlambda}
    }^2_{\mathrm{op}}
    +
    \norm{
      \mC^{-1}_{\vmu}
    }^2_{\mathrm{op}}
    \right)
    \, \norm{\vm_{\vlambda} - \vm_{\vmu} }_2^2
    \nonumber
    &&\quad\text{\textit{Triangle inequality}}
    \\
    &\;\geq
    -\frac{\alpha  \, (1-\alpha) \, }{2} \, \left( 2 \, M \right) \, \norm{\vm_{\vlambda} - \vm_{\vmu} }_2^2
    \nonumber
    &&\quad\text{\textit{Definition of \(\Lambda_{M}\)}}
    \\
    &\;\geq
    -\frac{\alpha \, (1-\alpha) \, }{2} \, \left( 2 \, M \right) \, \left( \norm{\vm_{\vlambda} - \vm_{\vmu} }_2^2 + \norm{\mC_{\vlambda} - \mC_{\vmu} }_F^2 \right)
    \nonumber
    \\
    &\;=
    -\frac{\alpha \, (1-\alpha) \, }{2} \, \left( 2 \, M \right) \, \norm{\vlambda - \vmu}_2^2
    \nonumber
  \end{alignat}
  which implies that \(q\) is  \( 2 \, M \)-strongly log-concave.
\end{proofEnd}

%%% Local Variables:
%%% TeX-master: "master"
%%% End:

